Teleoperation of Humanoid Robots: A Survey

Teleoperation of humanoid robots enables the integration of the cognitive skills and domain expertise of humans with the physical capabilities of humanoid robots. The operational versatility of humanoid robots makes them the ideal platform for a wide range of applications when teleoperating in a remote environment. However, the complexity of humanoid robots imposes challenges for teleoperation, particularly in unstructured dynamic environments with limited communication. Many advancements have been achieved in the last decades in this area, but a comprehensive overview is still missing. This survey paper gives an extensive overview of humanoid robot teleoperation, presenting the general architecture of a teleoperation system and analyzing the different components. We also discuss different aspects of the topic, including technological and methodological advances, as well as potential applications. A web-based version of the paper can be found at https://humanoid-teleoperation.github.io/.

==> sections/2-Background.tex <==
\section{Background}
\label{sec:Background}

% \subsection{Notation}
    % \item $\bm{1}_n$ and $\bm{0}_n$ denote the $n \times n$ identity and zero matrices in order.
    
% Frames are connected to physical reference points, and the coordinate system associated with the frames uniquely determine the position of the points in space.
% $\mathcal{I}$ denotes the inertial reference frame, where its $z$ axis pointing against the gravity.
% $ ^{\mathcal{A}}{\bm{R}}_\mathcal{B} \in SO(3)$ is the rotation matrix from frame $\mathcal{B}$ to frame $\mathcal{A}$. $^{\mathcal{A}}{\bm{p}}_\mathcal{I} \in \mathbb{R}^3$  and $^{\mathcal{B}}{\bm{p}}_\mathcal{I} \in \mathbb{R}^3$ denotes the displacement vectors from the inertial frame to the frames $\mathcal{A}$ and $\mathcal{B}$ respectively. We have $^{\mathcal{A}}{\bm{p}}_\mathcal{I} =  ^{\mathcal{A}}{\bm{R}}_\mathcal{B} \times ^{\mathcal{B}}{\bm{p}}_\mathcal{I}$.
    % \item $\text{sk}(\cdot) :\mathbb{R}^{3 \times 3} \to so(3)$ denotes \textit{skew-symmetric} operation of a matrix, such that given $\bm{A} \in \mathbb{R}^{3 \times 3}$, we have $\text{sk}(\bm{A}) := (\bm{A} - \bm{A}^\top)/2$.
    % \item $S(\cdot) :\mathbb{R}^{3} \to so(3)$ is the \textit{skew-symmetric} vector operation, such that given two vectors $\bm{a},\bm{b} \in \mathbb{R}^{3}$, it is defined as $\bm{a} \times \bm{b} = S(\bm{a})\bm{b}$.
    % \item  $\cdot^{\vee} : so(3) \to \mathbb{R}^{3}$ indicates the \textit{vee} operator, the inverse of the \textit{skew-symmetric} vector operator. Given a matrix $\bm{A} \in so(3)$ and a vector $\bm{b} \in \mathbb{R}^{3}$, it is defined as $\bm{A}\bm{b} = \bm{A}^{\vee} \times \bm{b}$.
    % \item The operator $\circ$ denotes the element-wise multiplication of two vectors or matrices.
% The L2-norm of the vector $\bm{a} \in \mathbb{R}^{n}$ is defined as $\left\lVert \bm{a} \right\rVert_2 = \sqrt{a_1^2+ \cdots +a_n^2}$.


\subsection{Modeling}


The human and the humanoid robot are modeled as multi-body mechanical systems with $n+1$ rigid bodies, called links, connected with $n$ joints each with one degree of freedom.
The configuration of a humanoid robot with $n$ joints depends on the robot shape, i.e., joint angles $\bm{s}\in \mathbb{R}^n$, and the position $^{\mathcal{B}}\bm{p}_{\mathcal{I}}\in \mathbb{R}^3$ and orientation $^{\mathcal{B}}{\bm{R}}_{\mathcal{I}}\in SO(3)$ of the floating base (usually associated with the pelvis) relative to the inertial or world frame $\mathcal{I}$. The robot configuration is indicated by $\bm{q} = (^{\mathcal{B}}\bm{p}_{\mathcal{I}}, ^{\mathcal{B}}{\bm{R}}_{\mathcal{I}}, s) \in \mathbb{R}^3 \times SO(3) \times \mathbb{R}^n$. The pose of a frame attached to a robot link $\mathcal{A}$ is computed via $(^{\mathcal{A}}\bm{p}_{\mathcal{I}}, ^{\mathcal{A}}\bm{R}_{\mathcal{I}}) = \bm{\mathcal{H}}_A(\bm{q})$, where   $\bm{\mathcal{H}}_A(\cdot) : \mathbb{R}^3 \times SO(3) \times \mathbb{R}^n \to \mathbb{R}^3 \times SO(3)$ is the geometrical forward kinematics.


The velocity vector $\bm{\nu} \in \mathbb{R}^3 \times \mathbb{R}^3 \times \mathbb{R}^n$ of the model is summarized in the vector $\bm{\nu}=(^{\mathcal{B}}\dot{\bm{p}}_{\mathcal{I}},^{\mathcal{B}}{\bm{\omega}}_{\mathcal{I}}, \dot{\bm{s}})$, where $^{\mathcal{B}}\dot{\bm{p}}_{\mathcal{I}}$,   $^{\mathcal{B}}{\bm{\omega}}_{\mathcal{I}}$ are the base linear and rotational (angular) velocity of the base frame, and $\dot{\bm{s}}$ is the joints velocity vector of the robot.
To compute the velocity of a frame $\mathcal{A}$ attached to the robot, i.e., $ ^{\mathcal{A}}\bm{v}_{\mathcal{I}}= (^{\mathcal{A}}\dot{\bm{p}}_{\mathcal{I}},^{\mathcal{A}}{\bm{\omega}}_{\mathcal{I}}) \in \mathbb{R}^{3} \times \mathbb{R}^{3}$, we have 
\begin{equation}
^{\mathcal{A}}\bm{v}_{\mathcal{I}}= \bm{\mathcal{J}}_A(\bm{q}) \bm{\nu}.
\label{eq:jacobian}
\end{equation}
$\bm{\mathcal{J}}_A(\bm{q}) \in \mathbb{R}^{6 \times (n+6)}$ is called the \textit{Jacobian} of the frame $\mathcal{A}$ and has the linear and angular part.


The dynamical model of the robot, with $n_c$ distinct reaction forces applied on the robot, is described by the equation:
\begin{equation}
\bm{M}(\bm{q}) \dot{\bm{v}} + \bm{C}(\bm{q},\bm{v})\bm{v} + \bm{g}(\bm{q}) = \bm{B}\bm{\tau} + \sum_{k=1}^{n_c}\bm{\mathcal{J}}_{k}^{T}(\bm{q})\bm{f}^{ext}_{k},
\label{eq:dyn}
\end{equation}
with $\bm{M}(\bm{q})$ being the symmetric positive definite inertia matrix of the robot, $\bm{C}(\bm{q},\bm{v})$ the vector of Coriolis and centrifugal terms, $\bm{g}(\bm{q})$ the vector of gravitational term, $\bm{B}=(\bm{0}_{n\times{6}},\bm{1}_n)^T$ a selector matrix, $\bm{\tau}$ the vector of actuator joint torques, $\bm{\mathcal{J}}_{k}(\bm{q})$ the Jacobian matrix associated with the application point of the $k$-th external force/torque, and $\bm{f}^{ext}_{k}$ the vector of the $k$-th external wrenches acting on the robot.
More information about the humanoid robot modeling can be found in \cite{sugihara2020survey} and \cite{marsden2013introduction}.

\subsection{Simplified Humanoid Robot Models}
Various simplified models are proposed in the literature in order to extract intuitive control heuristics and for real-time lower order motion planning.
Some of them include the Linear Inverted Pendulum Plus Flywheel \cite{pratt2006}, the Spring-Loaded Inverted Pendulum (SLIP) \cite{Wensing_SLIP},  the Cart-Table model \cite{Cart-Table}, the centroidal dynamics model \cite{orin2013centroidal}, and the single rigid-body model.
The most well-known approximation of the humanoid dynamics is the inverted pendulum model \cite{kajita20013d}.
% The humanoid dynamics can be approximated by an inverted pendulum,
In this model, the support foot (base joint) is connected to the robot center of mass (COM). Assuming the constant height of the inverted pendulum \cite{kajita20013d}, one can derive the equation of motion of the \textit{Linear Inverted Pendulum Model} (LIPM) by:
\begin{equation}
\ddot{\bm{x}} = \frac{g}{z_0}({\bm{x} - \bm{x}_{b}}),
\label{eq:lipm}
\end{equation}
where $g$ is the gravitational acceleration constant, $z_0$ is the constant height, $\bm{x} \in \mathbb{R}^2$ is the COM coordinate vector, and $\bm{x}_{b} \in \mathbb{R}^2$ is the base of LIPM coordinate vector.

The base of the LIPM is often assumed to be the Zero Moment Point (ZMP) (equivalent to the center of pressure, COP) of the humanoid robot \cite{vukobratovic1972stability}.
The LIPM dynamics can be divided to stable and unstable modes, where the unstable part is referred to (instantaneous) Capture Point \cite{pratt2006}, Divergent Component of Motion (DCM) \cite{takenaka2009real, englsberger2015}, or Extrapolated Center of Mass \cite{hof2008extrapolated} in the literature. The DCM dynamics is characterised by a first-order system as:
\begin{equation}
{\bm{\xi}} = \bm{x} + b{\bm{\dot{x}}},
\label{eq:dcmCOM}
\end{equation}
where $\bm{\xi}$ and $b = \sqrt{\frac{z_0}{g}}$ are the DCM variable and the time constant. This equation shows that the COM follows the DCM.
Differentiating \eqref{eq:dcmCOM} and replacing it to \eqref{eq:lipm} results to:
\begin{equation}
\dot{\bm{\xi}} = \frac{1}{b} (\bm{\xi}- \bm{x}_b).
\label{eq:dcm}
\end{equation}
This equation shows that DCM dynamics is unstable, i.e., it has strictly positive eigenvalue.
Equations \eqref{eq:dcmCOM} and \eqref{eq:dcm} together represents the dynamics of LIPM.
In the literature, the notion of DCM is used both for planning the footsteps and for stabilizing the robot motion. They will be explained in more detail in Section \ref{sec:RobotControl}.


% \todo[inline]{Joao: other relevant simple models include the Linear Inverted Pendulum Plus Flywheel \cite{pratt2006}, the Spring-Loaded Inverted Pendulum (SLIP)\cite{Wensing_SLIP},  the Cart-Table model \cite{Cart-Table}, the centroidal dynamics model, and the single rigid-body model. But we should probably not get into too much detail, just say these are used to extract intuitive control heuristics or for (real-time) lower order motion planing/mapping.} 




==> sections/4-RobotControl.tex <==
\section{Robot Control}
% \section{Humanoid Robot Retargeting and Control}
\label{sec:RobotControl}

\begin{figure*}[!t]
\centering
%\includegraphics[width=\textwidth]{Figures/section4/DRCControlArchitecture.pdf}
% \includegraphics[width=\textwidth]{Figures/section4/DRCControlArchitecture2.jpg}
% \includegraphics[width=\textwidth]{Figures/section4/CascadeControlArchitecture.pdf}
\includegraphics[width=\textwidth]{Figures/section3/retargeting-control-architecture.pdf}

\caption{Flowchart of a humanoid robot \modify{retargeting and} control architecture (red color references are coming from \modify{human interfaces}).}
\label{fig:controller_architecture}
\end{figure*}  


%   \todo[inline]{TODO. Rewrite section according to new structure}
% \todo[inline]{Kourosh: 
% Proposed structure for Section Robot Control: I think it is better to provide the methods for robot control in unilateral teleoperation scenarios here; and  we do not talk haptic feedback and the methods for providing haptic feedback to the user. In this section, we provide the information related to local or remote autonomy and control strategies of the robot.
% I'll suggest to do not use the term direct control, since in handbook of robotics, teleoperation section, the term direct control is used for lowest level of intelligence in teleoperation (the references are given to the robot without any modifications), while in our case, we update the given references.

% In this respect, I suggest:

% A. Simplified based control cascade architectures, where we have trajectory planner, simplified model control stabilizers, Whole-body QP controllers, ...


% B. Whole Body Controllers
% Inverse dyanmics, momentum based,...

% --
% Controller can get as input different types of commands from the retargeting block, e.g.,
% in Darvish2019 the com ref is given and the feet trajectory planner, .... are used for walking.
% In ishiguro 2018, instead the foot and com trajectories are given, and the stabilizer and IK are used in the control cascade architecture.
% }


%\begin{table*}[]
%     \center
%      \caption{Main work about the teleoperation of humanoid robots with associated control and perception methods}
%     \begin{tabular}{|c|c|c|c|}
%         \hline
%         Robot & Control & Perception & Ref.  \\
%         \hline
%          TORO & CoM-ZMP feedback controller + IK-based QP  & - & \cite{hu2014}\\
%          TORO & compliance momentum-based QP & task-relevant haptic feedback & \cite{abi2018}\\
%          TELESAR V & not specified & VR vision, audio, haptic primary colors & \cite{tachitelexistence}\\
%          JAXON & LIPM-based stabilizer + IK & VR vision & \cite{ishiguro2018}\\
%          Valkyrie  & momentum-based QP & GUI & \cite{jorgensen2019} \\
%          Atlas  & capturability-based & GUI & \cite{johnson2018}\\
%          HERMES  & contact force distribution & VR vision, haptic + balance feedback& \cite{ramos2018} \\
%          MAHRU  & MECoM + LIPM-based ZMP-feedback controller + IK & VR vision & \cite{kim2013} \\
%          HRP-2  & stabilizer + OSID-based QP & - & \cite{eramos2015}\\
%          HRP-2KAI  & LIPM-based ZMP-feedback + reactive step & GUI & \cite{cisneros2016}\\
%          HRP-4  & ID-based QP & - & \cite{difava2016}\\
%          DRC-HUBO  & compliance\&ZMP feedback controller + IK & GUI & \cite{zucker2015}\\
%          iCub & dynLIPM-based IS-MPC + IK-based QP & VR vision & \cite{penco2019}\\
%          iCub & LIPM-based DCM + IK-based QP & VR vision & \cite{elobaid2018}\\
%          iCub & momentum-based QP & - & \cite{darvish2019}\\
%          anonymous & RelaxedIK & - & \cite{rakita2019}\\
%          \hline
%     \end{tabular}
%     \label{tab:SOA}
% \end{table*}

% \begin{table*}[]
%     \center
%      \caption{Main work about whole-body teleoperation of humanoid robots and corresponding adopted control approaches.}
%     \begin{tabular}{|c|c|c|c|c|}
%         \hline
%         Ref. & Robot & Feedback Control & Low-Level Control & Command \\
%         \hline
%         \cite{hu2014} & TORO & MECoM-ZMP stabilizer & IK-based QP & joint position  \\
%         \hline
%         \cite{abi2018} & TORO & \multicolumn{2}{|c|}{compliance momentum-based QP} & torque \\
%         \hline
%         \cite{ishiguro2018} & JAXON & LIPM-based CoM-ZMP stabilizer & IK & joint position\\
%         \hline
%         \cite{jorgensen2019} & Valkyrie & \multicolumn{2}{|c|}{momentum-based QP + ID} & torque \\
%         \hline
%         \cite{johnson2017team} & Atlas  & \multicolumn{2}{|c|}{momentum-based QP + ID} & torque \\
%         \hline
%         \cite{ramos2018} & little HERMES  & \multicolumn{2}{|c|}{contact force distribution} & torque \\
%         \hline
%         \cite{kim2013} & MAHRU  & MECoM-ZMP LQR stabilizer & IK & joint position\\
%         \hline
%         \cite{eramos2015} & HRP-2 & commercial stabilizer & OSID-based QP & joint position \\
%         \hline
%         \cite{cisneros2016} & HRP-2KAI & LIPM-based CoM-ZMP stabilizer + reactive step & & joint position \\
%         \hline
%         \cite{difava2016} & HRP-4  & - & ID-based QP & joint position \\
%         \hline
%         \cite{zucker2015} & DRC-HUBO  & compliance + ZMP stabilizer & IK & joint position\\
%         \hline
%         \cite{penco2019} & iCub & dynLIPM-based IS-MPC & IK-based QP & joint position \\
%         \hline
%         \cite{elobaid2018a} & iCub & LIPM-based DCM stabilizer & IK-based QP & joint position \\
%         \hline
%         \cite{darvish2019} & iCub & \multicolumn{2}{|c|}{momentum-based QP} & torque \\
%         \hline
%     \end{tabular}
%     \label{tab:control}
% \end{table*}

%The term teleoperation most commonly refers to direct and continuous control of a robot. 
%The control strategy generally differs whether we teleoperate only upper-body movements (important for manipulation) or also leg motions, which are crucial for balancing and locomotion. In the following sections we examine both situations.
  


%   \todo[inline]{Sere: add a figure with the pyramid of Chris Atkeson about control (current consensus on whole-body control) but in form of cascade control architecture}


Humanoid robot control introduces many challenges to teleoperation scenarios.
For example, the robot model is nonlinear, hybrid, and underactuated with high degrees of freedom (DOFs).
The real robot dynamics also differs from its model in terms of link elasticity, joint backlash, and imperfect joint torque control tracking.
Moreover, even if we model the robot, the model of the environment (that the robot is interacting with) is not precise (partially known) and is subject to changes.
All these challenges entangled with the fact that the robot controller should run online, make the problem complicated.
% In this section, we describe in more detail these challenges and the proposed solutions in the literature.
Over the past decades, many control architectures have been proposed to teleoperate humanoid robots and to overcome the introduced challenges. Model-based optimal control architectures are the foremost technique used in the literature to address the problem of humanoid robot control. During DRC, most of the finalist control architectures converged to a similar design \cite{feng2015optimization, johnson2017team} where the robot trajectory planning and enhancing the robot stability is achieved by two different controller blocks. This architecture is conceptually demonstrated in Figure \ref{fig:controller_architecture}. This approach needs the humanoid's models (Section \ref{sec:Modeling}) as well as the references coming from the retargeting module.
% that is described in Section \ref{sec:Modeling}
% and the control details are described in Section
Control algorithms are described in Section \ref{sec:controllerArchitecture}.
More recently, different researchers try to solve the trajectory planing and enhancing the robot stability together 
% in a single control problem described in Section \ref{sec:ControlDesiderata}.
in a single control problem (Section \ref{sec:ControlDesiderata}).
% Moreover, the robot behavior is the interplay between highly dynamic motion (agility) versus stability and reliability of the robot motions.


% We have added the \textit{Path Planner} block to this architecture, in order to reconcile for teleoperation scenarios where a higher autonomy level is required.

\subsection{Modeling}
\label{sec:Modeling}
\subsubsection{Notations and complete humanoid robot models}
% \subsubsection{Notations and Humanoid Robot Models}
The human and the humanoid robot are modeled as multi-body mechanical systems with $n+1$ rigid bodies, called links, connected with $n$ joints, each with one degree of freedom.
The configuration of a humanoid robot with $n$ joints depends on the robot shape, i.e., joint angles $\bm{s}\in \mathbb{R}^n$, and the position $^{\mathcal{I}}\bm{p}_{\mathcal{B}}\in \mathbb{R}^3$ and orientation $^{\mathcal{I}}{\bm{R}}_{\mathcal{B}}\in SO(3)$ of the floating base (usually associated with the pelvis, ${\mathcal{B}}$) relative to the inertial or world frame $\mathcal{I}$\footnote{ With the abuse of notation, we will drop $\mathcal{I}$ in formulas for simplicity.}. The robot configuration is indicated by $\bm{q} = (^{\mathcal{I}}\bm{p}_{\mathcal{B}}, ^{\mathcal{I}}{\bm{R}}_{\mathcal{B}}, \bm{s}) \in \mathbb{R}^3 \times SO(3) \times \mathbb{R}^n$. The pose of a frame attached to a robot link $\mathcal{A}$ is computed via $(^{\mathcal{I}}\bm{p}_{\mathcal{A}}, ^{\mathcal{I}}\bm{R}_{\mathcal{A}}) = \bm{\mathcal{H}}_A(\bm{q})$, where   $\bm{\mathcal{H}}_A(\cdot) : \mathbb{R}^3 \times SO(3) \times \mathbb{R}^n \to \mathbb{R}^3 \times SO(3)$ is the geometrical forward kinematics.


The velocity vector $\bm{\nu} \in \mathbb{R}^{n+6}$ of the model is summarized in the vector $\bm{\nu}=(^{\mathcal{I}}\dot{\bm{p}}_{\mathcal{B}},^{\mathcal{I}}{\bm{\omega}}_{\mathcal{B}}, \dot{\bm{s}})$, where $^{\mathcal{I}}\dot{\bm{p}}_{\mathcal{B}}$,   $^{\mathcal{I}}{\bm{\omega}}_{\mathcal{B}}$ are the base linear and rotational (angular) velocity of the base frame, and $\dot{\bm{s}}$ is the joints velocity vector of the robot.
To compute the velocity of a frame $\mathcal{A}$ attached to the robot, i.e., $ ^{\mathcal{I}}\bm{v}_{\mathcal{A}}= (^{\mathcal{I}}\dot{\bm{p}}_{\mathcal{A}},^{\mathcal{I}}{\bm{\omega}}_{\mathcal{A}}) \in \mathbb{R}^{3} \times \mathbb{R}^{3}$, we have 
\begin{equation}
^{\mathcal{A}}\bm{v}_{\mathcal{I}}= \bm{\mathcal{J}}_A(\bm{q}) \bm{\nu}.
\label{eq:jacobian}
\end{equation}
$\bm{\mathcal{J}}_A(\bm{q}) \in \mathbb{R}^{6 \times (n+6)}$ is called the \textit{Jacobian} of $\mathcal{A}$ with the linear and angular parts.
Hence, the following affine relation between the robot velocity vector and  centroidal momentum, the whole-body momentum of a robot about its CoM, holds:
\begin{equation}
\bm{h}=\bm{A}(\bm{q})\bm{\nu},
\label{eq:CMM}
\end{equation}
%%
where $\bm{h} \in \mathbb{R}^{6}$. According to Newton-Euler's laws of motion and \eqref{eq:CMM}, the rate of change of centroidal momentum is \cite{orin2013centroidal}:
\begin{equation}
\begin{array}{c}
\dot{\bm{h}}
= \bm{A}\dot{\bm{\nu}}+\dot{\bm{A}}\bm{\nu} =\bm{f}^{g}+\sum_{i}\bm{\mathcal{J}}_{i}^{T}\bm{f}^{gr}_{i}+\sum_{j}\bm{\mathcal{J}}_{j}^{T}\bm{f}^{ext}_{i} \\
= \bm{f}^{g}+{\bm{\mathcal{J}}^{gr}}^{T}\bm{f}^{gr}+\sum_{i}\bm{f}^{ext}_{i}
\label{eq:eulermomentum}
\end{array}
\end{equation}
where $\bm{f}^g=(m\bm{g}^T, \bm{0}_{3\times{1}}^T)$
is the wrench due to gravity, $\bm{f}^{gr}_{i}$ and $\bm{f}^{ext}_{i}$ are the $i$'th ground reaction and other external wrenches applied to the robot, $\bm{\mathcal{J}}_{j}(\bm{q})$ the Jacobian matrix associated with the application point of the $k$-th external wrench.
All ground reaction wrenches $\bm{f}^{gr}$ have been written in a single matrix equation, with $\bm{\mathcal{J}}^{gr}$ being all the associated Jacobian matrices from the application points of the external ground reaction wrenches to the centroidal frame, the frame with the world orientation and the instantaneous CoM origin. %, and $\bm{f}^{gr}$ the vector of all the ground reaction wrenches.
%%
The $n+6$ equations of dynamical model of the robot, with all $n_c$ contact forces applied on the robot, is described by~\cite{cisneros2020inverse}:
\begin{equation}
\bm{M}(\bm{q}) \dot{\bm{\nu}} + \bm{C}(\bm{q},\bm{\nu})\bm{\nu} + \bm{g}(\bm{q}) = \bm{B}\bm{\tau} + \sum_{k=1}^{n_c}\bm{\mathcal{J}}_{k}^{T}(\bm{q})\bm{f}^{c}_{k},
\label{eq:dyn}
\end{equation}
with $\bm{M}(\bm{q})$ being the symmetric positive definite inertia matrix of the robot, $\bm{C}(\bm{q},\bm{\nu})$ the vector of Coriolis and centrifugal terms, $\bm{g}(\bm{q})$ the vector of gravitational terms, $\bm{B}=(\bm{0}_{n\times{6}},\bm{1}_n)^T$ a selector matrix, $\bm{\tau}$ the vector of actuator joint torques, and $\bm{f}^{c}_{k}$ the vector of the $k$-th contact wrenches acting on the robot.
More information about the humanoid robot modeling can be found in \cite{sugihara2020survey}. % marsden2013introduction}.


% \textcolor{blue}{According to Newton-Euler's laws of motion and \eqref{eq:dyn}, the rate of change of centroidal momentum, the whole-body momentum of humanoid robot about the CoM, is equal to the sum of all external wrenches applied to the robot:
% \begin{equation}
% \dot{\bm{h}}=\bm{f}_g+\sum_{i}\bm{f}_{gr,i}+\sum_{i}\bm{f}_{ext,i},
% \label{eq:eulermomentum}
% \end{equation}
% where $\bm{f}_g=(\bm{0}_{3\times{1}}^T,m\bm{g}^T)$
% is the wrench due to gravity, $\bm{f}_{gr,i}$ is the $i$'th ground reaction wrench exerted on the robot due to contact between these links and the environment, and the $\bm{f}_{ext,i}$ are other external wrenches applied to the robot. Since there is an affine relationship between the robot configuration space velocities and the robot's centroidal momentum, i.e.:
% \begin{equation}
% \bm{h}=\bm{A}(\bm{q})\bm{v},
% \label{eq:CMM}
% \end{equation}
% replacing \eqref{eq:CMM} into equation \eqref{eq:eulermomentum}, we have:
% \begin{equation}
% \bm{A}\dot{\bm{v}}+\dot{\bm{A}}\bm{v}=\bm{f}_g+\bm{Q}\bm{\rho}+\sum_{i}\bm{f}_{ext,i},
% \label{eq:eulermomentum1}
% \end{equation}
% where the sum of all ground reaction wrenches has been written in a single matrix equation, with $\bm{Q}$ being the transformation matrix from a task frame to the centroidal frame, the frame with the world orientation and the instantaneous COM origin, and $\bm{\rho}$ the vector of ground reaction wrenches expressed in the task frame.
% }


\subsubsection{Simplified humanoid robot models}
Various simplified models are proposed in the literature in order to extract intuitive control heuristics and for real-time lower order motion planning.
Some of them include the Linear Inverted Pendulum Plus Flywheel \cite{pratt2006}, the Spring-Loaded Inverted Pendulum (SLIP) \cite{Wensing_SLIP},  the Cart-Table model \cite{Cart-Table}, and the centroidal dynamics model \cite{orin2013centroidal}.
% , and the single rigid-body model.
The most well-known approximation of humanoid dynamics is the inverted pendulum model \cite{kajita20013d}.
% The humanoid dynamics can be approximated by an inverted pendulum,
In this model, the support foot (base joint) is connected through a variable length link to the robot center of mass (CoM). Assuming a constant height for the inverted pendulum \cite{kajita20013d}, one can derive the equation of motion of the \textit{Linear Inverted Pendulum Model} (LIPM) by:
\begin{equation}
\ddot{\bm{x}} = \frac{g}{z_0}({\bm{x} - \bm{x}_{b}}),
\label{eq:lipm}
\end{equation}
where $g$ is the gravitational acceleration constant, $z_0$ is the constant height, $\bm{x} \in \mathbb{R}^2$ is the CoM coordinate vector, and $\bm{x}_{b} \in \mathbb{R}^2$ is the base of the LIPM coordinate vector.

The base of the LIPM is often assumed to be the Zero Moment Point (ZMP) (equivalent to the center of pressure, CoP) of the humanoid robot \cite{vukobratovic1972stability}.
The LIPM dynamics can be divided into stable and unstable modes, where the unstable mode is referred as (instantaneous) Capture Point \cite{pratt2006}, Divergent Component of Motion (DCM) \cite{takenaka2009real, englsberger2015}, or Extrapolated Center of Mass \cite{hof2008extrapolated} in the literature. The stable mode is called Convergent Component of Motion (CCM) \cite{englsberger2015}. The DCM dynamics is characterised by a first-order system as:
\begin{equation}
{\bm{\xi}} = \bm{x} + b{\bm{\dot{x}}},
\label{eq:dcmCOM}
\end{equation}
where $\bm{\xi}$ and $b = \sqrt{\frac{z_0}{g}}$ are the DCM variable and the time constant. This equation shows that the CoM follows the DCM.
Differentiating \eqref{eq:dcmCOM} and replacing into \eqref{eq:lipm} results in:
\begin{equation}
\dot{\bm{\xi}} = \frac{1}{b} (\bm{\xi}- \bm{x}_b).
\label{eq:dcm}
\end{equation}
% This equation shows that DCM dynamics is unstable, i.e., it has a strictly positive eigenvalue.
Equations \eqref{eq:dcmCOM} and \eqref{eq:dcm} together represent the dynamics of LIPM.
In the literature, the notion of DCM is used both for planning the footsteps and for stabilizing the robot motion.
%  They will be explained in more detail in Section \ref{sec:RobotControl}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%% Simplified cascade %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cascade Control Architecture for Humanoid Robots}
\label{sec:controllerArchitecture}
% \todo[inline]{Luigi: I'd change this title with a more generic one, since this approach is not limited to DRC. smth like Simplified model based control for humanoid robots.}
% \todo[inline]{Kourosh: I partially agree with you, it is not limited to DRC. however, it does not mean necessarily simplified model are used! I updated the title, check if you like it otherwise, suggest a new one to discuss.}

The hierarchical control architecture is composed of \textit{Path and Footstep Planner}, \textit{Stabilizer}, \textit{Whole-Body Controller}, \textit{Low-level Joint Controller}, and \textit{State Estimator} as shown in Figure \ref{fig:controller_architecture}. %Each of these blocks will be discussed in more details in the rest of the section.
% The composition of \textit{Path and Footstep Planner} and \textit{Stabilizer} with a unifying approach as a single control problem is known as \textit{Motion Planning and High-level Controller} in the literature which will be discussed later in Section \ref{sec:MotionPlanning}. 
% \todo[inline]{Luigi: saying that they are referred to as a unified approach that is two separate names "Motion Planning" and "High-level Controller" is confusing. also the dedicated section has a different title "Motion Planning and Controller Desiderata". I would be more consistent with names.
% Anyways I would either not explain this at all since it is explained in section \ref{sec:MotionPlanning} or explain this better, since it is not clear form the sentence that in one case planner and stabilizer are separate blocks because based on a simplified model, while in the other they are embedded in a single optimization problem considering the whole robot dynamics. if I understood correctly.}
In general, as we go from left to right in the control pipeline, the robot model used in each block becomes more detailed, the receding horizon decreases, the frequency of the control loop increases, and lower-level input from the retargeting module is necessary.
The human operator can provide various reference inputs through the retargeting module (Section \ref{sec:Retargeting}) as shown in red in Figure \ref{fig:controller_architecture}.
% If the input is more on the left side of the figure, the expected level of autonomy from the robot increases.
As follows, each of these blocks is discussed.
%\todo[]{Luigi: limb poses can also be given without stabilizer if one uses a qp with proper task prioritizations in the wb control layer.   figure update}
%\todo[]{Kourosh: This is true, but from my point of view it leads to instability. However, I can mention that in the text or figure, and explain it.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Path and Footstep Planner}
\label{sec:PathandFootstepPlanner}
%Depending on the inputs provided by the retargeting module, different approaches have been proposed for the planning of the robot footsteps.
The goal of this block is to find the alternate footstep locations, moments, 
% instances (the moment which the robot makes contact with the environment),
and allocating a given footstep to the left or right foot to follow the user's commands. %\todo{Luigi: instances?}
% Another question which arises while solving this problem is related to contact sequencing, e.g., allocating a given footstep to the left or right foot.
% in order to perform agile motions, therefore contact planning is required for such scenarios,
% Even if the robot motion may involve hand contacts, here we mainly focus on footstep planning. 
The retargeting module may provide different types of input to the planner, such as the user's desired footstep contacts, the CoM velocity and the base rotational velocity, or the desired goal pose (region) in the workspace.
While with the first two inputs, the user is in charge of the obstacle avoidance, in the last one the planner deals with finding the whole path leading to the desired goal.
We structured this part of the section according to the category of the user's input.

% \textcolor{blue}{
% \textit{Input: Desired Footsteps}.
% The user provides the sequence of footstep locations or both the sequence of footstep locations and instances to the planner.
% % In case the sequence of footsteps location and instances are provided from the user.
% The footstep planner will modify the inputs such that it enhances the robot's stability and the feasibility of the task execution. An example of this footstep planner in teleoperation scenarios can be found in  \cite{ishiguro2018}, where the robot mimics the human foot motions. To do so, they have introduced the predicted support region where the robot DCM are kept inside that. Moreover, a delay is added to the DCM dynamics to increase the flexibility of the robot motion and enabling to perform dynamics teleoperated tasks.}
% \textcolor{blue}{
% Analogously, in \cite{johnson2017team} a footstep planning based on the human desired foot locations and adjustment to the ground using the perceived information of the environment was proposed. Later, the footstep locations were integrated with DCM dynamics in order to compute the footstep instance.
% In another example, the contact sequences and instances are fixed by the user offline \cite{caron2016multi}. 
% Conversely, in \cite{wiedebach2016walking} the robot steps on partial footholds with sharp surfaces, where the robot explores the contact line by rotating around it in order to identify the center of pressure. This results are used later in whole-body momentum algorithm blended with DCM dynamics in order to balance the robot with upper body angular momentum.
% }

\paragraph{Input: desired path or trajectory}
The role of the footstep 
% trajectory
planner is to find the sequence of foot locations and moments
% instances
given the CoM position or velocity, and the floating base orientation or angular velocity provided by \textit{Retargeting} module. %  \todo[inline]{Luigi: what do you mean desired path? is it a trajectory? referred to what entity? the line in between the feet?}
One possible approach to address this problem is based on the instantaneous capture point \cite{pratt2006}.
% Continuous renovation of footsteps enables high robustness to the disturbances acting on the robot.
Given the reference CoM position and velocity, one can compute the next 
% \todo{Luigi: why base?}base
foot contact point using the capture point relation in \eqref{eq:dcmCOM}.
In simple cases, the contact sequences can be preliminary identified by the user for example by a finite state machine, and the desired footstep locations are modified to the left or right side of the capture point according to the nature of the foot contact (left or right).
% the left or right foot \todo[inline]{Luigi: suggestion. I'd rather say according to the nature of the foot contact (left or right) instead of turn}turn.
% and conform to the ground.
Another way to find the sequence of footsteps is to formulate an optimization problem, where the cost function is decided based on commonsense heuristics.
\iffalse
\textcolor{blue}{For example in \cite{dafarra2018control} a trade-off between the footstep distance and instance for flat terrain is considered, whereas in \cite{garimort2011humanoid} the cost function includes the footstep length, obstacle avoidance, and the number of steps.}
\fi
The footstep 
% \todo{Luigi: I don't know about this term instance for footsteps. is it smth used in robotics?}instance
moment can be found from the CoM velocity such that the total gait cycle duration corresponds to the average CoM velocity and gait length. % \cite{siciliano2016springer}.


\paragraph{Input: desired goal region}
When the user provides the goal region, the humanoid robot not only should plan its footsteps but also should find a \textit{feasible} path for reaching the goal, if any exists. Different from wheeled mobile robots, feasible path here means an obstacle-free path or one where the humanoid robot can traverse the obstacles by stepping over.
Primary approaches for solving the integrated path and footstep planning problem are search-based methods and reactive methods.
% The reactive methods can be divided into optimization-based \cite{} and dynamical system approaches \cite{}.
The first step to find a feasible path is to perceive the workspace by means of the robot perception system, finding the regions where the robot can step. Following the identification of the workspace, a feasible path is planned.

Search-based algorithms try to find a path from the starting point to the goal region by searching a graph. The graph can be made using a grid map of the environment or by a random sampling of the environment.
Some of the methods used in the literature to perform footstep planning are A* \cite{chestnutt2005footstep, griffin2019footstep}, D* Lite \cite{garimort2011humanoid}, RRT variations \cite{perrin2011fast}, and dynamic programming techniques \cite{kuffner2001footstep}.
The \textit{completeness}, \textit{global optimality}, and the ability of real-time \textit{replanning} of the path in dynamic environments are the important features of these search-based algorithms when selecting.
% On the other hand, the search-based approaches depend on a predefined set of actions to be taken when passing from one node or vertex to another one in the graph.
These algorithms are not very efficient for real-time execution when an exhaustive search is done, hence, to enhance the efficiency a \textit{heuristic} is chosen in order to prune the search space and perform a greedy search.
% The choice of the heuristic becomes of paramount importance for finding and tailoring an optimal path while respecting the humanoid's constraints \cite{}.


% As mentioned before, the footstep planning problem has been addressed as an optimization problem as well. In \cite{herdt2010online} the problem has been formulated with a model predictive control (MPC) approach, allows finding the foot poses as a continuous decision making problem by formulating it as a quadratic programming (QP) optimization problem.
The reactive methods for footstep planning problem can be addressed as an optimization problem or a dynamical system as well.
In \cite{herdt2010online} the problem has been devised as a Model Predictive Control (MPC) approach. It allows finding the foot poses as a continuous decision making problem by formulating it as a Quadratic Programming (QP) optimization problem.
However, when the footstep rotation or the obstacle-avoidance is added to the problem, the optimization problem becomes non-convex, therefore, there is no guarantee on completeness and global optimality \cite{deits2014footstep}. In order to relax the non-convex constraints, \cite{deits2014footstep} transformed footstep rotations into a set of approximated functions, and obstacle-avoidance constraints are transformed into a set of obstacle-free regions with convex shapes. As a result, they have formulated the optimization problem as a mixed-integer quadratic programming problem.
% \textcolor{blue}{A similar approach for finding the hand contact location has been carried out by \cite{mason2018mpc} as well.}
However, the main limitation of this approach is its high computational complexity.
%, i.e., they cannot be solved in real-time currently.
In this context, the problem of path planning and obstacle avoidance for a humanoid robot can be viewed as a simplified dynamical system control approach, for example, by using potential fields \cite{fakoor2015revision}. %\cite{hong2010evolutionary, fakoor2015revision}.% solved the obstacle avoidance problem with 
% In this context, the problem of path planning for a humanoid robot can be viewed as a simplified dynamical system control approach. For example, \cite{hong2010evolutionary, fakoor2015revision} solved the obstacle avoidance problem with potential fields.
% \cite{dafarra2018control} employed a simplified unicycle model, or \cite{lavalle2001randomized} solved the planning problem with the kinodynamic approach.
% \todo[inline]{Luigi: I think this footstep/path planning part can be shortened to 15-20 lines. We could simply indicate the different approaches and when to use them with few citations without going into too many details.}
% Another approach to find the footstep location is to provide the footstep locations automatically by searching the workspace for horizontal planes reachable by the robot. In these cases, the duration of the walking cycle can be defined by the user or found by some heuristics rules, or found by solving an optimization problem \cite{}.

% \todo[inline]{Kou: contact wrench cone stability criteria , Hirukawa2006, Wieber 2002}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Stabilizer}
\label{sec:Stabilizer}
The main goal of the stabilization layer is to implement a control law that enhances the stability of the centroidal dynamics of the robot. Because of the complexity of robot dynamics, classical approaches are limited to examine the stability of a closed-loop control system.
% Because of the However, the humanoid robot dynamics is nonlinear, underactuated, and hybrid, in which they limit the use of classical approaches to examine the stability of the closed-loop controlled system.
% To overcome\todo{Luigi: missing object of verb}
Therefore, other insights such as ZMP criteria and DCM dynamics are tailored in order to evaluate how far the robot is about to fall \cite{koolen2012}.
The \textit{stabilizer} gets as input the reference poses for the end-effectors such as head, arms, and feet, together with the desired CoM trajectory. These inputs are provided by the retargeted human motion and/or by the \textit{Path and Footstep  Planner}.
However, these reference trajectories may destabilize the robot behavior, therefore the \textit{stabilizer} adapts the references according to the stability criteria.
%\textcolor{blue}{, ensuring the stability of the system.}
% given the current situation.
Depending on the lower level whole-body controller, the output of the \textit{stabilizer} are modified references for the CoM pose, the end-effector poses, the contact points, the contact wrenches and/or the rate of change of the momenta.
% In the following
Next, we provide an overview of controllers according to different stability criteria adopted so far.
%to stabilize the control references.

% Because of complexity of the robot model, conventional stabilization approaches recur to a simplified model of the robot such as the LIPM as described in Section \ref{sec:Background}. Different approaches in the literature are proposed for controlling the robot such that it does not fall. In the rest of this part, we try to provide an overview of them assuming the simplified robot model unless it is mentioned.

% \begin{figure}[!t]
% \centering

% \begin{subfigure}[b]{\columnwidth}
% \includegraphics[width=\columnwidth]{Figures/section4/ZMPController2.jpg}
% \caption{}
% \label{fig:ZMPcontroller}
% \end{subfigure}

% \begin{subfigure}[b]{\columnwidth}
% \includegraphics[width=\columnwidth]{Figures/section4/DCMZMPController2.jpg}
% \caption{}
% \label{fig:DCMZMPcontroller}
% \end{subfigure}

% \begin{subfigure}[b]{\columnwidth}
% \includegraphics[width=\columnwidth]{Figures/section4/ContactForceBalanceController2.jpg}
% \caption{}
% \label{fig:ContactForceBalanceController}
% \end{subfigure}
% \caption{Different stability criteria controllers. a) ZMP controller; b) DCM-ZMP controller; c) contact wrench controller.}
% \label{}
% \end{figure} 

\begin{figure}[!t]
\centering

\includegraphics[width=\columnwidth]{Figures/section4/StabilizerControllers.pdf}

\caption{Different stability criteria controllers. a) ZMP controller; b) DCM-ZMP controller; c) contact wrench controller.}
\label{fig:StabilizerControllers}
\end{figure} 

% \begin{figure}[!t]
% \centering
% %\includegraphics[width=\columnwidth]{Figures/section4/DCMZMPController.pdf}
% \includegraphics[width=\columnwidth]{Figures/section4/DCMZMPController2.jpg}
% \caption{Schematic architecture for DCM-ZMP controller.}
% \label{fig:DCMZMPcontroller}
% \end{figure}  

% \begin{figure}[!t]
% \centering
% %\includegraphics[width=\columnwidth]{Figures/section4/ContactForceBalanceController.pdf}
% \includegraphics[width=\columnwidth]{Figures/section4/ContactForceBalanceController2.jpg}
% \caption{Schematic architecture for contact wrench controller.}
% \label{fig:ContactForceBalanceController}
% \end{figure} 

\paragraph{ZMP controller}
These controllers are based on the idea that the robot's ZMP should remain inside the support polygon of the base \cite{vukobratovic1972stability, koolen2012}, as shown in Figure \ref{fig:StabilizerControllers}.
%\ref{fig:ZMPcontroller}. 
Given the footstep trajectories provided by the planner or the human, this module computes the desired ZMP.
% An approach to design the desired ZMP trajectory is to divide the walking into two phases of the single and double support.
While walking, in single support the desired ZMP remains in the middle of the support polygon (e.g., left foot), during double support the desired ZMP moves smoothly from the previous support leg to the middle of the new support leg polygon (e.g., from the left foot to the right foot).
% This pattern is repeated continuously while walking.
Following that, a ZMP controller makes sure the real ZMP tracks the desired ZMP trajectory.
% , by reducing the error between the real and desired ZMP values. 
% Following that, the desired COM motion will be generated using \eqref{eq:lipm} such that the error on ZMP converges to zero.
In order to converge the ZMP error to zero, the desired CoM motion (using \eqref{eq:lipm}) or the desired foot force distribution is computed \cite{choi2007, kajita2010}. %kajita2014introduction, 
The ZMP controller can be based on PID, pole placement, optimal controllers, or other control approaches.
The real ZMP is estimated using the Force/Torque sensors located at the robot heel.
% \textcolor{blue}{ In Figure \ref{fig:ZMPcontroller}, the lower level controllers refer to the whole-body and low-level joint controllers in Figure \ref{fig:controller_architecture}.}
To avoid the phase delay of the ZMP tracking due to the mechanical compliance and control \cite{kajita2010}, one can model the delay and consider it in the ZMP controller.
% one can model the delay and formulate the ZMP controller as a MPC problem.
% A detailed description of controllers based on ZMP stability criteria and their implementation on real robots can be found in \cite{choi2007, kajita2014introduction, kajita2010}.
% ZMP controller has been adopted for humanoid robot teleoperation scenarios as well. 
% Examples of ZMP controller with LIPM assumption can be found in \cite{hu2014, kim2013}, where the human footsteps are captured and imitated by the robot.
% Then to achieve a more human-like behavior, also the motion similarity in the joint space is treated, with particular focus on a knee stretched walking and human-like swing leg motions. The resulting redundant inverse kinematics problem is formulated as a QP with dynamic equality and inequality constraints. 
% The CoM-ZMP stabilizer proposed by Choi \textit{et al.} \cite{choi2007}, which relies on the concept of motion-embedded CoM (MECoM) Jacobian, has also been adopted to teleoperate the robot MAHRU in \cite{kim2013}, which first proposed a simultaneous assignment of upper-body tasks and walking motion. The online footprint imitation is realized by feeding the recognized and adapted human step parameters into a classical ZMP based walking controller.
Nevertheless, the ZMP controller introduces several limitations.
If the robot is subject to high disturbances, it does not adapt online to footstep locations to avoid the robot from falling.
% Because of pre-computed footstep location, it does not provide the ability to the robot to reactively and online adapts or replan its footsteps in order to compensate high disturbances acting on the robot.
% Moreover, it is hard to extend this approach to non-flat terrain or when the support foot rotates or slides.
Moreover, this approach hardly extends to non-flat terrain or when the support foot rotates or slides.

% Finally, this approach is limited in non-flat terrain and the cases which the support foot rotates or moves. Moreover, in teleoperation scenarios, if the robot imitates the human leg motion, the human footstep is intrinsically variable and therefore unknown a priori.
% \textcolor{blue}{To overcome the footstep adjustment in case of disturbances, the idea of instantaneous Capture Point is firstly introduced in \cite{pratt2006}.}
% and later the Divergent Component of Motion (DCM) in 3-D terrain \cite{takenaka2009real, englsberger2015} is presented in the literature.




\paragraph{DCM-ZMP controller}
% and the Capture Point (CP) \cite{koolen2012}, in order to find feasible CoM trajectories. These models  have  become  very  popular  after  the introduction of the ZMP as a stability criterion.
Another approach that is often employed with the simplified model control is the DCM \cite{takenaka2009real}, which can be viewed as an extension of the capture point concept to the three-dimensional case for uneven terrain \cite{englsberger2015}.
Equation \eqref{eq:dcm} shows that the DCM dynamics is unstable, i.e., it has a strictly positive eigenvalue, and using equation of LIPM \eqref{eq:lipm} it can be shown that the CoM dynamics converges to the DCM value.
% As formulated in Section \ref{sec:Modeling}, the DCM dynamics \eqref{eq:dcm} is unstable, and using equation of LIPM \eqref{eq:lipm} it can be shown that the COM dynamics converges to DCM value.
Therefore, the main goal of this controller is to implement a control law that stabilizes the unstable DCM dynamics \eqref{eq:dcm} as well as the ZMP as mentioned previously.
To stick to the formulation presented in \ref{sec:Modeling}, the DCM-ZMP controller is explained with flat pavement assumption, however, for the extension of the controller to 3D, one can check \cite{englsberger2015}.
The block diagram of the DCM-ZMP stabilizer is shown in Figure \ref{fig:StabilizerControllers}.
% \ref{fig:DCMZMPcontroller}.
Based on the desired footstep, the desired DCM and its derivative are extracted. Later, we close the loop on the desired DCM in order to stabilize its dynamics by:
\begin{equation}
\dot{\bm{\xi}} -\dot{\bm{\xi}}_{ref} = - k_{\xi} ({\bm{\xi}} -{\bm{\xi}}_{ref}),
\label{eq:dcmController}
\end{equation}
where $k_{\xi}>0$.
\iffalse
\textcolor{blue}{so that the error on DCM error converges to zero asymptotically.}
\fi
By replacing \eqref{eq:dcmController} into equation \eqref{eq:dcm}, the desired ZMP is found by:
\begin{equation}
\bm{zmp}_{ref}= \bm{\xi} - b \dot{\bm{\xi}}_{ref} + b k_{\xi} ({\bm{\xi}} -{\bm{\xi}}_{ref}),
\label{eq:dcmZMPController}
\end{equation}
and the external forces acting on the robot can be found by \eqref{eq:lipm}. Finally, the desired values are provided to the ZMP Controller.
One can formulate both the DCM and ZMP controllers together in a single optimal control problem as well \cite{cisneros2020inverse}.
% \textit{\textbf{Simplified Model Control Stabilization}}.  
% The  motion  of  the  robot  can  be viewed considering  the linear momentum dynamics only 
% \begin{equation}
% \dot{\bm{h}}_l=m\ddot{\bm{x}}+\sum_{k=1}^{n_c}\bm{f}_{k}^l+m\bm{g}
% \label{eq:linmomentumdyn}
% \end{equation}
% where $\bm{x}$ represents the position of the CoM and $\bm{f}_{k}^l$ the linear component of the external force acting on the system and $\dot{\bm{h}}_l$ the rate of change of the linear centroidal momentum.
% The DCM is given by \cite{englsberger2015}:
% \begin{equation}
% \bm{\xi} = \bm{x} + b \dot{\bm{x}}
% \label{eq:dcm}
% \end{equation}
% where $b$, in case of constant CoM height $z0$, is the pendulum time constant, i.e. $b=\sqrt{z0/g}$.
% Using (\ref{eq:linmomentumdyn}) and (\ref{eq:dcm}), the DCM time derivative is given by:
% \begin{equation}
% \dot{\bm{\xi}} = \frac{1}{b}(\bm{\xi} - \bm{x})+\frac{b}{m}\sum_{k=1}^{n_c}\bm{f}_{k}^l
% \label{eq:dcmd}
% \end{equation}
% By introducing the virtual repellent point (VRP) as
% \begin{equation}
% \bm{r}^{vrp}=\bm{x}-\frac{b^2}{m}\left(\sum_{k=1}^{n_c}\bm{f}_{k}^l+\bm{g}\right)=\bm{x}-\frac{\dot{\bm{h}}_lb^2}{m}
% \label{eq:vp}
% \end{equation}
% Eq. (\ref{eq:dcmd}) can be simplified as:
% \begin{equation}
% \dot{\bm{\xi}} = \frac{1}{b}(\bm{\xi} - \bm{r}^{vrp}).
% \label{eq:dcmdvp}
% \end{equation}
% The main goal of the stabilization layer is to implement a control law that stabilizes the unstable DCM dynamics (\ref{eq:dcmdvp}).
% To  guarantee  the  tracking  of  the  desired  DCM  trajectory the following control law is chosen:
% \begin{equation}
% \bm{r}^{vrp}_{des}=\bm{\xi}_{ref} + b \dot{\bm{\xi}}_{ref}+\bm{K}^{\xi}(\bm{\xi} + \bm{\xi}_{ref}).
% \label{eq:dcmlaw}
% \end{equation}
% By using the control input (\ref{eq:dcmlaw}) in (\ref{eq:dcmdvp}), one has:
% \begin{equation}
% \dot{\bm{\tilde{\xi}}} = \dot{\bm{\xi}} - \dot{\bm{\xi}}_{ref} = \frac{1}{b} (\bm{I}_3-\bm{K}^{\xi})\bm{\tilde{\xi}}.
% \label{eq:dcmlaw1}
% \end{equation}
% The choice of $\bm{K}^{\xi} > \bm{I}_3$ guarantees an asymptotically stable closed loop error dynamics.
% \textcolor{blue}{
% This simplified model control stabilization is adopted in \cite{elobaid2018a,darvish2019}, then feeding a low-level control layer, framed as QP, which guarantees the tracking of the robot’s reference trajectories, organized as a hierarchy of tasks.
% Also in \cite{jorgensen2019}, the walking behavior is based on the ideas of CP. Concretely, the instantaneous capture point (ICP) is planned using \cite{seyde2018}, which is then used to compute the desired momentum rate for the QP.} %This CP-based walking has useful stability properties that are used to monitor the safe execution of trajectories and pause potentially unsafe walking trajectories.
% \textcolor{red}{
% Feedback controllers (or stabilizers) have been used not only to guarantee the balance but also to give some compliance to the robot motion and lessen the severity of impacts between the robot and the environment \cite{zucker2015, abi2018}. In \cite{abi2018}, the compliance controller is topped with a higher level position/velocity whole-body motion one, allowing the user to design a controller for a force/torque compliance controlled robot from a pre-designed and tuned compliance controller without having to deal with its specificities. Their control algorithm, once again, computes a suitable set of balancing wrenches by solving a QP.}
%As the user gets closer to reach the robot constraints, her/his commands are gradually scaled down to zero in order to ensure the stability of the system.
% \textcolor{red}{
% In this case a feedback controller is usually employed to correct the control references to work against many existing disturbances in the real robot system \cite{hu2014,zucker2015,cisneros2016,ishiguro2018}.}
% DCM-ZMP controller has been deployed for retargeting of the human feet motion to the robot feet motion in \cite{ishiguro2018}.
DCM-ZMP controller has been deployed for whole-body retargeting in \cite{ishiguro2018}.
% They have added some safety constraints to the reference human footsteps in order to enhance the stability of the system.
In order to enhance the stability of the system, the authors have introduced the predicted support region where the robot time-delayed DCM is kept inside that region.
% An example of this footstep planner in teleoperation scenarios can be found in  \cite{ishiguro2018}, where the robot mimics the human foot motions. To do so, they have introduced the predicted support region where the robot DCM are kept inside that. Moreover, a delay is added to the DCM dynamics to increase the flexibility of the robot motion and enabling to perform dynamics teleoperated tasks.

% \textcolor{blue}{
% When trying to make the robot imitate the human stepping, the impact force at the ground on the humanoid robot's foot can be a serious external disturbance. In \cite{ishiguro2018}, Ishiguro \textit{et al.} implement a safety mechanism for a soft and safe ground contact, by setting a vertical velocity limitation that is proportional to the foot height. 
% After processing the human input references, they modify end-effector poses and CoM position to preserve the robot balance and feed them into an IK solver. The resulting joint angles are then stabilized by using a bipedal feedback controller \cite{kajita2010}, which acts as an external disturbance absorber using the feet force sensors values and reference ZMP trajectories. With this method, the robot JAXON has been successfully teleoperated while high-kicking or hitting a tennis ball with a racket.}




%%%%%%%%%%%%%%%%% 


\paragraph{Contact wrench controller}
This controller finds the desired contact wrenches at each contact point such that it enhances the robot stability. A schematic block diagram of this controller is shown in Figure \ref{fig:StabilizerControllers}.
This controller has been initially introduced in \cite{ott2011} and later considered by \cite{hirukawa2006universal} as a stability augmentation criteria when introducing the contact constraints. This approach is similar to the momentum-based controller and will be explained in more detail later. However, to be thorough, we have mentioned it here as well.

\iffalse
% \ref{fig:ContactForceBalanceController}.
Given the reference CoM position $\bm{x}_\mathcal{COM}^{d}$ and velocity $\dot{\bm{x}}_\mathcal{COM}^{d}$, and the reference base $\mathcal{B}$ orientation and angular velocity, \cite{ott2011},
% englsberger2014overview} 
a PD compliance control finds the net desired external wrench vector $\bm{w}_{ext}^{d}$ by:
\begin{equation}
\begin{array}{c}
\bm{w}_{ext}^{d}= \begin{bmatrix}
m\bm{g}\\ 
\bm{0}
\end{bmatrix}  
- \bm{K}_D
\begin{bmatrix}
\dot{\bm{x}}_\mathcal{COM} -\dot{\bm{x}}_\mathcal{COM}^{d} \\ 
\tau_D( \bm{\omega}_\mathcal{B}^{d}  ,\bm{\omega}_\mathcal{B} )
\end{bmatrix} 
\\
- \bm{K}_P
\begin{bmatrix}
{\bm{x}}_\mathcal{COM} -{\bm{x}}_\mathcal{COM}^{d} \\ 
{\tau_P({ {\bm{R}}_\mathcal{B}^{d},{\bm{R}}_\mathcal{B})}} 
\end{bmatrix}, 
\label{eq:ExternalWrenchDesired}
\end{array}
\end{equation}
where $\bm{K}_P$ and $\bm{K}_D$ are the symmetric positive semi-definite proportional and damping gain matrices; $\tau_P$ and $\tau_D$ functions compute the error on the rotational term of the base orientation error.
% In this equation,
In \eqref{eq:ExternalWrenchDesired}, the first term compensates gravity.
Given the contact points, the desired net wrenches at the robot CoM are employed to compute the wrench at each contact point.
% Using the desired net wrenches acting on the robot COM and given the contact points, the wrench at each contact point is computed.
% It is assumed that the contacts points are known, for example by using the ZMP controller or DCM-ZMP controller provided previously.
% In \cite{ott2011}, frictional grasping problem and an optimization problem are solved in order to calculate the desired contact wrenches.
% The desired contact wrenches in \cite{ott2011} is calculated  based on frictional grasping problem is proposed by \cite{ott2011} where an optimization problem is defined.
 An approach to compute the desired contact wrenches based on the frictional grasping method is proposed by \cite{ott2011} where an optimization problem is defined.
Here without the loss of generality, only the forces at the contact points are considered.
A \textit{contact map} matrix $\bm{G}_{c} \in \mathbb{R}^{6 \times 3c}$ is identified to map $c$ contact force vectors $\bm{f}_c$ to the net wrench at CoM by:
\begin{equation}
    \bm{w}_{ext} = \bm{G}_c \bm{f}_c.
    \label{eq:contactMap}
\end{equation}
Using this equation and given the $\bm{w}^d_{ext}$ from \eqref{eq:ExternalWrenchDesired}, an optimization problem is defined  to compute the contact forces:
\begin{equation}
\begin{array}{c}
\text{arg~}\underset{\bm{f}_c}{\text{min}}
~( \bm{Q}_\mathcal{COM} \| \bm{F}^d_{\mathcal{COM},ext}-\bm{G}_{c, f} \bm{f}_c \|^{2}+\\
\bm{Q}_\mathcal{B} \| \bm{\tau}^d_{\mathcal{B},ext}-\bm{G}_{c,\tau} \bm{f}_c \|^{2}+
\bm{R} \| \bm{f}_c \|^{2}), \\
 s.t. ~~ {f}_{c,z} \ge 0,\\
({f}_{c,x})^2 + ({f}_{c,y})^2 \le \mu({f}_{c,z})^2,
\end{array}    
    \label{eq:contactOptimization}
\end{equation}
the first term in this equation tracks the COM position with the highest priority, the second term tracks of the base rotational motion, and the last term with the lowest priority is the regularization term.
% the first term in this equation is related to tracking the COM position with the highest priority, the second term is related to tracking of the base rotational motion, and the last term with the lowest priority is the regularization term.
$\bm{G}_{c, f}$ and $\bm{G}_{c,\tau}$ in \eqref{eq:contactOptimization} are related to the linear and rotational terms of $\bm{G}_{c}$.
 The optimization is subject to unilateral friction and the friction cone constraints.
 These constraints have been considered as a stability criterion in \cite{ hirukawa2006universal}. % wieber2002stability,
The desired contact forces are later passed to the whole-body controller in order to compute the joint torques.
\fi
% Anoteher initrpossible control strategy is to adopt a posture and balance controller based on contact force optimization \cite{ott2011}. After defining the net forces and moments the robot must apply on its own CoM in order to follow the reference human motion, the knowledge of the contact state (single or double support) is used to generate the proper force distribution to each leg (or other contact points, if available). The robot follows the human movements while maintaining balance by controlling the interaction forces between its contacting points and the environment. The solution is found analytically using heuristics for simple contact cases or via numerical optimization when there are multiple contact points.
% \textcolor{red}{In their bilateral system, Ramos \textit{et al.} \cite{ramos2018} use the first strategy to dynamically teleoperate the robot little HERMES to take steps.}
% \todo[inline]{Luigi: also this part about the stabilizer can be condensed in 15-20 lines. especially the a. subsubsection can be shortened.}

\subsubsection{Whole-Body control layer (WBC)}

This block provides the reference joint angles, velocities, accelerations and/or torques to the low-level joint controller.
% or from the retargeting module. 
% It should be noted that, if the end-effector values are passed to this module without the checks in \textit{Stabilizer}, it can degrade the performance of the whole controller, i.e., resulting to failures.
% It gets as input the reference poses of the head, arms, feet end-effectors from the higher-level controller. Moreover, the references for CoM positions, and contact points and wrenches are transferred to this module as well. Alternatively, the reference rate of change of momentum can be passed to this module as well.
It gets as input the retargeted human references together with the planner references, both corrected by the stabilizer.
% \todo[inline]{Luigi: what about reference joint angles? add also in fig 5. I would simply say: It takes as input the retargeted human references together with the planner references, both corrected by the stabilizer.}
% \textcolor{blue}{Within this block, the inverse kinematics (IK) and/or inverse dynamics (IK) problem are defined and solved.
% The outputs of this block are the vector of joint angles, velocities, acceleration, or the joint torques or a mixture of them.} 
In the following, different approaches of the whole-body control are presented.

\paragraph{Whole-Body inverse instantaneous velocity kinematics control}
The problem of inverse instantaneous or velocity kinematics is to find the configuration state velocity vector $\bm{\nu}(t)$ for a given set of task space velocities using the Jacobian relation as in \eqref{eq:jacobian}.
One common approach is to formalize the controller as a constrained  QP problem with inequality and equality constraints.
The problem can be formulated as:
\begin{equation}
\begin{array}{c}
\text{arg~}\underset{\bm{\nu}}{\text{min}} \underset{k}{\sum} w_k( \| \bm{A}_{k}\bm{\nu}-\bm{b}_{k}\|^{2})+ \epsilon\| \bm{\nu}\|^{2}, \\
 s.t. 
          \quad \bm{d}_{min} \le \bm{D}\bm{\nu} \le \bm{d}_{max}, \\
           \quad\quad\quad \bm{\nu}_{min} \le \bm{\nu} \le \bm{\nu}_{max}, \\
\end{array}
\label{eq:ivkqp}
\end{equation}
where $\bm{\nu}$ is the joint velocities control input vector; $\bm{A}_k$ is the equivalent Jacobian matrix of the task $k$ governed by \eqref{eq:jacobian}; $\bm{b}_k$ is the reference velocity value for the task, $\epsilon$ is a regularization factor used to handle singularities.
% where $\bm{\nu}$ refers to the joint velocities control input vector; $\bm{A}_k$ the equivalent Jacobian matrix of the task $k$ governed by \eqref{eq:jacobian}; $\bm{b}_k$ the reference velocity value for the task, $\epsilon$ the regularization factor used to handle singularities.
$\bm{\nu}_{min}$ and $\bm{\nu}_{max}$ are the control input limits, and $~\bm{d}_{min} \le \bm{D}\bm{\nu} \le \bm{d}_{max}~$ are other equality and inequality constraints, e.g., collision avoidance or contact related constraints.
% High priority tasks can be regarded as equality constraints while lower priority tasks can be considered in the cost function with relative weight $w_k$.
% When teleoperating only the upper-body of a humanoid robot, while maintaining the lower limbs fixed, the control can be simply formulated as an Inverse Kinematics (IK) problem with references also computed at a kinematic level.
Conventional solutions of redundant inverse kinematics are founded on the pseudo-inverse of the Jacobian matrix \cite{kanoun2011}.
% , where lower priority tasks are projected into the null space of the higher priority tasks
% \cite{kanoun2011}.
% Although being naive, this approach can be very effective for manipulation tasks as demonstrated in \cite{gitai} by GITAI, a robotics startup developing technology for mobile-based humanoid telepresence in space.
%\todo[]{Luigi: these two paragraphs use basically the same equation. Also I don't get the conceptual difference between a. and b. I suggest mergin ghte two paragraphs in one, only using (\ref{eq:ivkqp}) where b is not only the task space ref but it can be also a joint posture ref. and in that case A=I. }
%\todo[]{Kourosh: They are different problem however sounds similar. Their methods to solve them are different also.}
\paragraph{Whole-Body inverse kinematics control}
The problem of Inverse Kinematics (IK) is to find the configuration space vector $\bm{q}(t)$ given the reference task space poses.
This problem can be solved analytically, however, this solution is not scalable to different robots and for a humanoid robot with a high degree of freedom is not feasible.
Differently from inverse instantaneous velocity kinematics, to solve the IK problem a nonlinear constrained optimization problem is defined as:
% A common approach to solve the IK problem is to define a nonlinearly constrained optimization problem as:
\begin{equation}
\begin{array}{c}
\text{arg~}\underset{\bm{q}}{\text{min}} \underset{k}{\sum} w_k~ dist(\bm{\mathcal{H}}_{k}(q),\bm{x}^d_{k})^{2}+ \epsilon\| \bm{q}\|^{2}, \\
 s.t. 
          \quad \bm{d}_{min} \le \bm{D}\bm{q} \le \bm{d}_{max}, \\
           \quad\quad\quad \bm{q}_{min} \le \bm{q} \le \bm{q}_{max}, \\
\end{array}
\label{eq:ikqp}
\end{equation}
which uses the geometrical forward kinematics relation $\bm{\mathcal{H}}_{k}(q)$ of task $k$ to minimize the distance with respect to the task goal pose $\bm{x}^d_k$.
Residual function $dist(.)$ in this equation is defined as Euclidean distance for position task and inverse skew-symmetric vector of $\bm{\mathcal{H}}_{k}(q)^{T}  {}^{\mathcal{I}}\bm{R}_{k}$ for the rotational task.
% However,
Solving this problem might be time-consuming and the results can be discontinuous as well.
To solve this problem, a common approach in the literature is to transform the whole-body IK into a whole-body inverse velocity kinematics problem.
% whereby the optimization problem is linear with a quadratic form.
\iffalse
\textcolor{blue}{In order to compute the reference value $\bm{b}_k$ in \eqref{eq:ivkqp}, a dynamical system is defined as $\bm{b}_k={\bm{v}}^d_k+\lambda\bm{e}_k$ value for the $k$-th task, with ${\bm{v}}^d_k$ being the feed-forward reference velocity term, $\lambda$ the convergence error gain, and $\bm{e}_k$ the residual vector between current and goal poses \cite{rapetti2019model}.}
\fi

\paragraph{Whole-Body inverse dynamics control}
The Inverse Dynamics (ID) refers to the problem of finding the joint torques of the robot to achieve the desired motion given the robot's constraints such as joint torque limits and feasible contacts.
There are different techniques to solve the ID problem in the literature \cite{righetti2012quadratic}.
A common situation is to minimize the torques and joint accelerations of the robot for achieving the desired references,
%contact wrench or end-effector pose \todo[inline]{Luigi: I would say to achieve the desired references in general, since the reference are not limited to end effector poses but also to other links and also to joints},
without violating the robot constraints.
To reach the desired end-effector poses and contact wrenches, one can realize it based on the following optimization problem:
\begin{subequations} \label{eq:idqp}
\begin{align}
& \text{arg~}\underset{\bm{\tau}}{\text{min}}~ \underset{k}{\sum} w_k (\|\ddot{\bm{x}}_{k}-\ddot{\bm{x}}^d_{k}\|^{2})+ \epsilon\| \bm{\tau}\|^{2}\nonumber\\
& ~~~~~~ + \underset{i}{\sum} w'_i (\|{\bm{f}_{C,i}}-{\bm{f}}^d_{C,i}\|^{2}),\label{eq:idqp_min}\\
&  s.t.~~~\bm{\tau}_{min} \le \bm{\tau} \le \bm{\tau}_{max}, \label{eq:idqp_TConst}\\
& \bm{d'}_{min} \le \bm{D'}\dot{\bm{\nu}} \le \bm{d'}_{max}, \label{eq:idqp_AccConst}\\
& \bm{J}_C\dot{\bm{\nu}}+\dot{\bm{J}}_C\bm{\nu}=0,  \label{eq:idqp_fixedFoot}\\
& \bm{f}_{C} \ge 0, \label{eq:idqp_contact}
% & {f}_{C,z} \ge 0, \label{eq:idqp_NoPull}\\
% & ({f}_{C,x})^2 + ({f}_{C,y})^2 \le \mu({f}_{C,z})^2,\label{eq:idqp_FricCone}
\end{align}
\end{subequations}
% \todo[]{Rafael: It is actually very difficult to solve the optimization problem expressed like this" }
% \todo[]{Kourosh: do you have any suggestion to write the constraints in another form.}
% \begin{align*}
% \vspace{-5pt}
% \begin{array}{c}
%  ~~~~~~~s.t.~~~
%         \bm{M}\dot{\bm{v}} + \bm{C}\bm{v} + \bm{g} = \bm{B}\bm{\tau} + \sum\bm{J}^{T}\bm{f}_{ext}~~~~~~~~~~(\ref{eq:dyn})
% \end{array}
% \end{align*}
% \begin{equation}
% \vspace{-5pt}
% \label{eq:tlimit}
% \begin{array}{c}
% \bm{\tau}_{min} \le \bm{\tau} \le \bm{\tau}_{max}
% \end{array}
% \end{equation}
% \begin{equation}
% \vspace{-5pt}
% \label{eq:vellimit}
% \begin{array}{c}
%           \frac{\bm{v}_{min}-\bm{v}}{\Delta t} \le \dot{\bm{v}} \le \frac{\bm{v}_{max}-\bm{v}}{\Delta t}
% \end{array}
% \end{equation}
% \begin{equation}
% \vspace{-5pt}
% \label{eq:plimit}
% \begin{array}{c}
%           \frac{\bm{q}_{min}-\bm{q}-\bm{v}\Delta t}{\frac{1}{2}\Delta t^2} \le \dot{\bm{v}} \le \frac{\bm{q}_{max}-\bm{q}-\bm{v}\Delta t}{\frac{1}{2}\Delta t^2}
% \end{array}
% \end{equation}
% \begin{equation}
% \vspace{-5pt}
% \label{eq:contact}
% \begin{array}{c}
%          \bm{J}_C\dot{\bm{v}}+\dot{\bm{J}}_C\bm{v}=0
% \end{array}
% \end{equation}
% \begin{equation}
% \vspace{-5pt}
% \label{eq:frictioncone}
% \begin{array}{c}
%           \bm{f}_C \ge 0
% \end{array}
% \end{equation}
% \begin{equation}
% \vspace*{0.5 cm}
% \label{eq:autocollision}
% \vspace{-5pt}
% \begin{array}{c}
%           \ddot{d}(b_1,b_2) \ge \frac{1}{\Delta t}(-\lambda \frac{d(b_1,b_2)-\delta_s}{\delta_i-\delta_s}-\dot{d}(b_1,b_2) )
% \end{array}
% \end{equation}
where $\ddot{\bm{x}}^{d}_{k}$ is the reference value for the motion task expressed in accelerations and ${\bm{f}^{d}_{C,i}}$ is the desired contact wrench given the dynamics equation of motion of the robot in \eqref{eq:dyn}, \eqref{eq:idqp_TConst} is the torque limits, \eqref{eq:idqp_AccConst} is the general constraints such as velocity and joint angle limits, and collision avoidance limits expressed with joint acceleration vector, \eqref{eq:idqp_fixedFoot} is the non-sliding contact constraint, and \eqref{eq:idqp_contact} is the constraint of  foot contacts.
% \eqref{eq:idqp_NoPull} is the unilateral constraint of the foot contacts, and \eqref{eq:idqp_FricCone} is the foot friction cone constraint. 
% A detailed explanation 
The details of the constraints can be found~\cite{difava2016, righetti2012quadratic}.
% , (\ref{eq:autocollision}) the
% collision-avoidance constraint between body $b_1$ and $b_2$ of the robot or the environment, with distance between the two bodies $d(b_1,b_2)$, damping coefficient $\lambda$, security distance $\delta_s$ and influence distance $\delta_i$. 

% The inverse dynamics (ID) approach \eqref{eq:idqp} has been proposed in \cite{difava2016} to handle multi-contact teleoperated motions on the HRP-4 robot.  The reference values can alternatively be expressed in the task space, recurring to operational-space inverse dynamics (OSID), which has been proposed for teleoperating the HRP-2 robot in \cite{eramos2015}, during a live performance consisting of fine balanced captured dance movements. In this work, the OSID control, framed as a hierarchical QP, handles the effects of the dynamics in feed-forward, with a feedback loop coming from the commercial stabilizer of HRP-2, which controls the movements of the flexible parts of the feet according to the measurements of the ankle force-torque sensors.

% \textcolor{blue}{In order to compute the joint reference commands, the robot's states are required. In this case, the state estimator through the forward kinematics and dynamics will provide these values.
% Moreover, the robot joints can be controlled in different modes, therefore a mixture of both whole body inverse dynamics and kinematics can be used in order to control the robot motion.
% Finally, in equations \eqref{eq:ivkqp} and \eqref{eq:idqp} the reference velocity and acceleration values can be computed by defining a dynamical equation on the error between the robot end-effector pose and desired robot end-effector poses. An example of such definition of such dynamical equation can be found in \cite{rapetti2019model}.}

\iffalse
This controller finds the desired contact wrenches at each contact point such that it enhances the robot stability. A schematic block diagram of this controller is shown in Figure \ref{fig:StabilizerControllers}.
% \ref{fig:ContactForceBalanceController}.
Given the reference CoM position $\bm{x}_\mathcal{COM}^{d}$ and velocity $\dot{\bm{x}}_\mathcal{COM}^{d}$, and the reference base $\mathcal{B}$ orientation and angular velocity, \cite{ott2011},
% englsberger2014overview} 
a PD compliance control finds the net desired external wrench vector $\bm{w}_{ext}^{d}$ by:
\begin{equation}
\begin{array}{c}
\bm{w}_{ext}^{d}= \begin{bmatrix}
m\bm{g}\\ 
\bm{0}
\end{bmatrix}  
- \bm{K}_D
\begin{bmatrix}
\dot{\bm{x}}_\mathcal{COM} -\dot{\bm{x}}_\mathcal{COM}^{d} \\ 
\tau_D( \bm{\omega}_\mathcal{B}^{d}  ,\bm{\omega}_\mathcal{B} )
\end{bmatrix} 
\\
- \bm{K}_P
\begin{bmatrix}
{\bm{x}}_\mathcal{COM} -{\bm{x}}_\mathcal{COM}^{d} \\ 
{\tau_P({ {\bm{R}}_\mathcal{B}^{d},{\bm{R}}_\mathcal{B})}} 
\end{bmatrix}, 
\label{eq:ExternalWrenchDesired}
\end{array}
\end{equation}
where $\bm{K}_P$ and $\bm{K}_D$ are the symmetric positive semi-definite proportional and damping gain matrices; $\tau_P$ and $\tau_D$ functions compute the error on the rotational term of the base orientation error.
% In this equation,
In \eqref{eq:ExternalWrenchDesired}, the first term compensates gravity.
Given the contact points, the desired net wrenches at the robot CoM are employed to compute the wrench at each contact point.
% Using the desired net wrenches acting on the robot COM and given the contact points, the wrench at each contact point is computed.
% It is assumed that the contacts points are known, for example by using the ZMP controller or DCM-ZMP controller provided previously.
% In \cite{ott2011}, frictional grasping problem and an optimization problem are solved in order to calculate the desired contact wrenches.
% The desired contact wrenches in \cite{ott2011} is calculated  based on frictional grasping problem is proposed by \cite{ott2011} where an optimization problem is defined.
 An approach to compute the desired contact wrenches based on the frictional grasping method is proposed by \cite{ott2011} where an optimization problem is defined.
Here without the loss of generality, only the forces at the contact points are considered.
A \textit{contact map} matrix $\bm{G}_{c} \in \mathbb{R}^{6 \times 3c}$ is identified to map $c$ contact force vectors $\bm{f}_c$ to the net wrench at CoM by:
\begin{equation}
    \bm{w}_{ext} = \bm{G}_c \bm{f}_c.
    \label{eq:contactMap}
\end{equation}
Using this equation and given the $\bm{w}^d_{ext}$ from \eqref{eq:ExternalWrenchDesired}, an optimization problem is defined  to compute the contact forces:
\begin{equation}
\begin{array}{c}
\text{arg~}\underset{\bm{f}_c}{\text{min}}
~( \bm{Q}_\mathcal{COM} \| \bm{F}^d_{\mathcal{COM},ext}-\bm{G}_{c, f} \bm{f}_c \|^{2}+\\
\bm{Q}_\mathcal{B} \| \bm{\tau}^d_{\mathcal{B},ext}-\bm{G}_{c,\tau} \bm{f}_c \|^{2}+
\bm{R} \| \bm{f}_c \|^{2}), \\
 s.t. ~~ {f}_{c,z} \ge 0,\\
({f}_{c,x})^2 + ({f}_{c,y})^2 \le \mu({f}_{c,z})^2,
\end{array}    
    \label{eq:contactOptimization}
\end{equation}
the first term in this equation tracks the COM position with the highest priority, the second term tracks of the base rotational motion, and the last term with the lowest priority is the regularization term.
% the first term in this equation is related to tracking the COM position with the highest priority, the second term is related to tracking of the base rotational motion, and the last term with the lowest priority is the regularization term.
$\bm{G}_{c, f}$ and $\bm{G}_{c,\tau}$ in \eqref{eq:contactOptimization} are related to the linear and rotational terms of $\bm{G}_{c}$.
 The optimization is subject to unilateral friction and the friction cone constraints.
 These constraints have been considered as a stability criterion in \cite{ hirukawa2006universal}. % wieber2002stability,
The desired contact forces are later passed to the whole-body controller in order to compute the joint torques.
\fi


\paragraph{Momentum-based control} This controller finds the configuration space acceleration and ground reaction forces such that the robot follows the given desired rate of change of whole-body momentum \cite{orin2013centroidal, cisneros2020inverse}. % koolen2016
% Also momentum-based controller can be designed in a QP fashion\cite{koolen2016}.
% According to Newton-Euler's laws of motion and \eqref{eq:dyn}, the rate of change of centroidal momentum, the whole-body momentum of humanoid robot about the CoM, is equal to the sum of all external wrenches applied to the robot:
% \begin{equation}
% \dot{\bm{h}}=\bm{f}_g+\sum_{i}\bm{f}_{gr,i}+\sum_{i}\bm{f}_{ext,i},
% \label{eq:eulermomentum}
% \end{equation}
% where $\bm{f}_g=(\bm{0}_{3\times{1}}^T,m\bm{g}^T)$ is the wrench due to gravity, $\bm{f}_{gr,i}$ is the $i$'th ground reaction wrench exerted on the robot due to contact between these links and the environment, and the $\bm{f}_{ext,i}$ are other external wrenches applied to the robot. Since there is an affine relationship between the robot configuration space velocities and the robot's centroidal momentum, i.e.:
% \begin{equation}
% \bm{h}=\bm{A}(\bm{q})\bm{v},
% \label{eq:CMM}
% \end{equation}
% replacing \eqref{eq:CMM} into equation \eqref{eq:eulermomentum}, we have:
% \begin{equation}
% \bm{A}\dot{\bm{v}}+\dot{\bm{A}}\bm{v}=\bm{f}_g+\bm{Q}\bm{\rho}+\sum_{i}\bm{f}_{ext,i},
% \label{eq:eulermomentum1}
% \end{equation}
% where the sum of all ground reaction wrenches has been written in a single matrix equation, with $\bm{Q}$ being the transformation matrix from a task frame to the centroidal frame, the frame with the world orientation and the instantaneous COM origin, and $\bm{\rho}$ the vector of ground reaction wrenches expressed in the task frame.
Using \eqref{eq:eulermomentum}, one can formulate the following QP optimization problem:
\begin{equation}
\begin{array}{c}
\text{arg}~\underset{\dot{\bm{\nu}}_d,\bm{\rho}}{\text{min}}~(\bm{A}\dot{\bm{\nu}}_d-\bm{b})^T\bm{C}_h(\bm{A}\dot{\bm{\nu}}_d-\bm{b}) \\
+ {\bm{f}^{gr}}^T\bm{C}_{gr}\bm{f}^{gr} + \dot{\bm{\nu}}_d^T\bm{C}_{\dot{\nu}}\dot{\bm{\nu}}_d\\
 s.t.
        %   \bm{A}\dot{\bm{v}}_d+\dot{\bm{A}}\bm{v}=\bm{f}_g+\bm{Q}\bm{\rho}+\sum_{i}\bm{f}_{ext,i}~~~(\ref{eq:eulermomentum1}) \\
           \quad\quad\quad \bm{f}^{gr}_{min} \le \bm{f}^{gr} \le \bm{f}^{gr}_{max} 
\end{array}
\label{eq:QPmomentum}
\end{equation}
where $\bm{C}_{h}$, $\bm{C}_{gr}$ and $\bm{C}_{\dot{\nu}}$ are weighting matrices and $\bm{b}=\dot{\bm{h}}_d-\dot{\bm{A}\bm{\nu}}$, with $\dot{\bm{h}}_d$ being a desired rate of change of centroidal momentum. Finally, the \textit{pre-specified} external wrenches $\bm{f}^{ext}_{i}$, the \textit{computed} $\bm{f}^{gr}{i}$ ground reaction wrenches, and the \textit{computed} joint accelerations $\dot{\bm{\nu}}_d$ are used with an inverse dynamics algorithm to compute the robot joint torques.

% This approach has been adopted to teleoperate through user interfaces both the Atlas and Valkyrie robots \cite{johnson2018,jorgensen2019}. As well in \cite{darvish2019}, Darvish \textit{et al.} propose the use of a momentum-based control but for the teleoperation of the iCub robot during single support motions. The control problem is formulated as QP optimization problem to achieve the two tasks of maintaining the balance and following the retargeted human posture, while carefully monitoring and regulating the contact wrenches, considering the associated feasible domains.


% \textit{\textbf{Quadratic Program Control}}
% In the case of whole-body teleoperation, one of the main challenges is to control the robot in a way that guarantees its dynamical balance while trying to follow the retargeted human references.
% The dynamics of the robot (or of a simplified model of the robot) has to be taken into consideration in --at least-- either the computation of the reference trajectories (Section \ref{sec:TeleoperationSystemDevices}), or in the control law.
% One common approach is to formalize the controller as a constrained quadratic programming (QP) problem with inequality and equality constraints, comprising (\ref{eq:dyn}), where the references are the (retargeted) human inputs.
% The QP formalism can be applied to different types of control   \cite{hu2014,abi2018,jorgensen2019,difava2016,penco2019,darvish2019}. The generic QP formulation is indeed: 
% \begin{equation}
% \begin{array}{c}
% \underset{\bm{u}}{\text{minimize}}~f(\bm{u})=\underset{k}{\sum} w_k( \| \bm{A}_{k}\bm{u}-\bm{b}_{k}\|^{2})+ \epsilon\| \bm{u}\|^{2} \\
%  s.t. 
%           \quad \bm{\underline{d}} \le \bm{D}\bm{u} \le \bm{\overline{d}} \\
%           \quad\quad\quad \bm{u}_{min} \le \bm{u} \le \bm{u}_{max} \\
% \end{array}
% \label{eq:QP}
% \end{equation}
% where $\bm{u}$ is the control input vector, which can be the joint velocities $\bm{v}$, the joint acceleration $\bm{\dot{v}}$ or torques $\bm{\tau}$; $\bm{A}_k$ is the equivalent Jacobian matrix of the task $k$; $\bm{b}_k$ the reference value for the task coming from the master operator, $\epsilon$ a regularization factor used to handle singularities, $\bm{u}_{min}$ and $\bm{u}_{max}$ the control input limits and $~\bm{\underline{d}} \le \bm{D}\bm{u} \le \bm{\overline{d}}~$ are other equality and inequality constraints, e.g. dynamics, collision avoidance, or contact related constraints. High priority tasks can be regarded as equality constraints while lower priority tasks can be considered in the cost function with relative weight $w_k$.

% The choice of tasks is generally standard. The position of the ground projection of the center of mass is taken into consideration to encode the balance of the robot. Since the distribution of mass of the human operator could differ significantly from the robot, a reference height of the waist (that can be easily scaled to fit the equivalent value for the robot) is usually preferred to a center of mass one. Cartesian tasks to control the pose of a specific link are widely used. The end-effectors poses are essential to perform any manipulation or locomotion tasks. To provide more stability, a task concerning the orientation of the floating base is commonly included in the controller. Alternatively, the orientation of other links, such as the head or the chest, can  be considered. If controlling the momentum of the robot, also the rate  of change
% of  centroidal  momentum has to be taken into account as a task.

% A typical choice of the task priorities is to give the highest priority to the contact related tasks (e.g. feet pose while standing) and CoM related tasks. Then the other tasks act in the null-space of the former with the end-effectors having a higher relative weight $w_k$ over other tasks like the orientation of a specific link. Optimization approaches can be used to find automatically the best priorities \cite{penco2020}.

% \textit{\textbf{Inverse Kinematics Control with Stabilizer}}.
% An alternative to torque control is to control the robot in position casting a IK-based QP to compute the joint angles commands:
% \begin{equation}
% \begin{array}{c}
% \underset{\bm{v}}{\text{minimize}}~\underset{k}{\sum} w_k( (\bm{J}_{k}\bm{v}-\bm{b}_{k})^T\bm{C}_q(\bm{J}_{k}\bm{v}-\bm{b}_{k})+\bm{v}^T\bm{C}_{\epsilon}\bm{v}) \\
%  s.t. 
%           \quad \bm{\underline{d}} \le \bm{D}\bm{v} \le \bm{\overline{d}} \\
%           \quad\quad\quad \bm{v}_{min} \le \bm{v} \le \bm{v}_{max} \\
% \end{array}
% \label{eq:QP}
% \end{equation}
% where $\bm{C}_q$ and $\bm{C}_\epsilon$ are positive definite cost matrices and $\bm{b}_k=\dot{\bm{p}}_d+\lambda\bm{e}$ is the reference value for the $k$-th task, with $\dot{\bm{p}}_d$ being the feed-forward velocity term, $\lambda$ the convergence error gain and $\bm{e}$ the Cartesian pose error.


\paragraph{Other control formalisms}
The whole-body control problem can be formalized with different cost functions and solving a QP problem at each control cycle to compute the optimal control inputs is not the only viable solution. Indeed, other approaches such as Linear Quadratic Regulator (LQR) \cite{mason2014, kuindersma2016optimization} and MPC \cite{ kelly2017introduction, posa2014direct} % borrelli2017, rao2009survey, 
have been utilized as well. % in the literature

% \begin{comment}
\iffalse
\textcolor{blue}{
\textit{Linear Quadratic Regulator (LQR)}. An alternative can be to rely on a full-state LQR, using the robot dynamics \cite{mason2016}. LQR is essentially an automated way of finding an appropriate state-feedback controller. The robot model in (\ref{eq:dyn}) is linearized by determining a linear time-invariant (LTI) or linear time-varying system.
% of the form:
% \begin{equation}
% \dot{\bm{x}} = \bm{A}\bm{x}+\bm{B}\bm{u},
% \label{eq:lti}
% \end{equation}
% where $\bm{x}$ is the state of the system, $\bm{u}$ the input, $\bm{A}$ the state matrix and $\bm{B}$ the input matrix.
LQR leads to an optimization problem in the state space in the form of:
\begin{equation}
\begin{array}{c}
\underset{\bm{u}}{\text{arg~min}}~\mathlarger{\int_{0}^{\infty}}(\bm{x}^T\bm{Q}\bm{x}+ \bm{u}^T\bm{R}\bm{u})dt, \\
\end{array}
\label{eq:LQR}
\end{equation}
where $\bm{x}$ and $\bm{u}$ are the system state and input vector, and $\bm{Q}$ and $\bm{R}$ are the regularization gains for the states and inputs.
The solution to LQR is:
\begin{equation}
\begin{array}{c}
\bm{\tau}=\bm{\tau}_0-\bm{K}\bm{x} ,
\end{array}
\label{eq:LQRsol}
\end{equation}
where $\bm{\tau}_0$ is the vector of joint torques that compensates the dynamics of the robot around the linearized state and $K$ is found by solving the continuous-time Riccati differential equation combined with the system dynamics. The second term in \eqref{eq:LQRsol} is associated with the input vector $\bm{u}$ which minimizes the feedback control law.
% \textcolor{blue}{The rigid contact constraints are embedded in the linearized dynamics by projecting the linearized system into the nullspace of the constraint matrix using the projection matrix, where it leads to an optimization problem in the reduced state space.}
Some examples of the LQR method to control humanoid robots can be found in \cite{mason2014}, \cite{kuindersma2016optimization}.}
% It is possible to optimize for elements in the task space defined as a linear combination of the original state vector, and choose the task space objectives to be
% the regulation of the CoM and total momentum or other references coming from the master operator \cite{mason2014}.


% , e.g. the gravity compensation term for a linearization at zero velocity poses.
% The rigid contact constraints 
% \begin{equation}
% \left[  \begin{array}{cc} \bm{J}_c & \bm{0}\\ [1pt]
%  \dot{\bm{J}}_c & \bm{J}_c 
% \end{array}  \right]
% \left[  \begin{array}{c} \bm{v} \\ [1pt]
%  \dot{\bm{v}} \end{array}  
% \right] = \left[  \begin{array}{c} \bm{0} \\ [1pt]
%  \bm{0} \end{array}  
% \right],
% \end{equation} are embedded in the linearized dynamics by projecting the linearized system into the nullspace of the constraint matrix using the projection matrix $N$.
% This leads to an optimization problem in the reduced state space:
% \begin{equation}
% \begin{array}{c}
% \underset{\bm{u}}{\text{minimize}}~\mathlarger{\int_{0}^{\infty}}(\bm{x}_m^T\bm{Q}_m\bm{x}_m+ \bm{u}^T\bm{R}\bm{u})dt \\
% \end{array}
% \label{eq:LQR}
% \end{equation}
% where $\bm{x}_m=\bm{N}^T\bm{x}$, $\bm{A}_m=\bm{N}^T\bm{A}\bm{N}$, $\bm{B}_m=\bm{N}^T\bm{B}$  and $\bm{Q}_m=\bm{N}^T\bm{Q}\bm{N}$.
% The feedback control law that minimizes the value of the cost is: 
% \begin{equation}
% \begin{array}{c}
% \bm{u}=-\bm{K}_m\bm{x} \\
% \end{array}
% \label{eq:LQRsol}
% \end{equation}
% where $\bm{K}_m$ is given by: 
% \begin{equation}
% \begin{array}{c}
% \bm{K}_m= \bm{R}^{-1}(\bm{B}_m^T\bm{P}(\bm{t})\bm{N}^T)\\
% \end{array}
% \label{eq:LQRK}
% \end{equation}
% and $\bm{P}$ is found by solving the continuous time Riccati differential equation.
% By mapping the gains $\bm{K}_m$ from the minimal system back to the full system, we obtain the control for the humanoid robot
% \begin{equation}
% \begin{array}{c}
% \bm{\tau}=\bm{\tau}_0-\bm{K}\bm{x} ,
% \end{array}
% \label{eq:LQRsol1}
% \end{equation}
% where $\bm{\tau}_0$ is the vector of joint torques that compensates the dynamics of the robot around the linearized state, e.g. the gravity compensation term for a linearization at zero velocity poses.
% It is possible to optimize for elements in the task space defined as a linear combination of the original state vector, and choose the task space objectives to be
% the regulation of the CoM and total momentum or other references coming from the master operator \cite{mason2014}.


\textcolor{blue}{
\textit{Model Predictive Control (MPC)}.
% Another control strategy that can be adopted to teleoperate humanoid robots is model predictive control (MPC). MPC 
It is a suite of optimization-based control techniques applied to dynamical systems. MPC controllers optimize an objective function based on a predicted evolution of the system states in the future \cite{borrelli2017}.
In a linear case, the prediction model is:
\begin{equation}
\begin{cases} 
\bm{x}_{k+1}=\bm{A}\bm{x}_{k}+\bm{B}\bm{u}_{k} \\
\bm{y}_{k}=\bm{C}\bm{x}_{k},
\end{cases}
\label{eq:mpc1}
\end{equation}
where $\bm{x}_k$, $\bm{u}_k$ and $\bm{y}_k$ are respectively the state, the input and the output of the system at time $k$.
An approach to relating the input and the current state vector can be formulated as:
\begin{equation}
\bm{x}_{k}=\bm{A}^k\bm{x}_{0}+\sum_{j=0}^{k-1}\bm{A}^j\bm{B}\bm{u}_{k-1-j}.
\label{eq:mpc2}
\end{equation}
The goal is to solve the following optimization problem, finding the optimal sequence of control inputs:
\begin{equation}
\begin{array}{c}
\underset{\bm{u}_0, ..., \bm{u}_{N-1} }{\text{arg~min}}~\bm{x}_N^T\bm{P}\bm{x}_N+\sum_{k=0}^{N-1}\bm{x}_k^T\bm{Q}\bm{x}_k+\bm{u}_k^T\bm{R}\bm{u}_k,\\
 s.t. 
           \quad\quad \bm{\dot{x}} - \bm{f}(\bm{x}, \bm{u})=\bm{0},\\ \quad\quad \bm{g}((\bm{x}, \bm{u})) \le \bm{0},\\ 
           \quad\quad \bm{h}((\bm{x}, \bm{u})) = \bm{0},
\end{array}
\label{eq:mpc3}
\end{equation}
where $\bm{R}$ is a positive definite matrix and $\bm{Q}$ and $\bm{P}$ are positive semi-definite matrices. 
Moreover, the MPC problem is accompanied by a set of constraints including the robot dynamics constraint (the first constraint in \eqref{eq:mpc3}), inequality constraints such as joint position, velocity and torque limits, contact unilaterality and friction cone constraints, and finally equality constraints such as  non-sliding contact constraints.
In order to solve \eqref{eq:mpc3}, the optimal control problem %of  \todo{Luigi: "it" refers to what?} it
is transformed into an algebraic nonlinear programming problem, namely called a transcription process \cite{kelly2017introduction, rao2009survey}.
To do that, two categories of shooting methods and direct methods are utilized in the literature. While the shooting method searches for input variable values and uses the forward simulation results to compute the cost of trajectory, the direct method finds the input and state variable simultaneously without explicit simulation.
The multiple shooting method blends these two approaches together \cite{posa2014direct}.
However, the main limitation of MPC approach for humanoid robot control is the computational cost of solving the optimization problem.
Therefore, the use of MPC in real-time is typically not straightforward and it is usually convenient to recur to a simplified prediction model.}
\fi
% Generally for robot walking the LIPM, or extended versions of it \cite{pratt2006,scianca2020}, are adopted.
% In \cite{penco2019} for example, the iCub robot has been teleoperated recurring to a MPC \cite{scianca2020} to generate the swing foot and CoM trajectories during walking, with the operator imparting a direction and velocity references for the humanoid gait through the analog sticks. In the proposed framework the human operator can also choose to fully control the robot in real-time when performing manipulation tasks. In this case the retargeted human references are corrected by a simple ZMP-based stabilizer. The operator can select one of the two modalities by using the buttons of the VR controller. Both share the same low-level controller, formalized as an IK-based QP, for computing in real time the joint commands to be sent to the robot. 
% MPC approaches are not limited only to walking motions but can also be applied to different whole-body movements \cite{koenemann2015}, given some knowledge about the reference trajectory of the task that will be performed.


\subsubsection{Low-level Joint Controller}
One of the main challenges in deploying a humanoid robot controller is the different behavior obtained in simulation and on the real robot of the low-level joint torque tracking.
The low-level joint controller is in charge of generating motor commands to ensure the tracking of the higher-level control inputs.
The input to the joint controller can be the desired joint positions, velocities, torques, or a mixture of them. The output of this controller is the current or voltage to the motors driving the joints.
While the joint position can be directly measured by the encoder sensors, the joint velocity feedback is obtained by differentiating in time the encoder values, hence it can be noisy. Joint torque sensors or whole-body estimation algorithms equipped with distributed joint-torque sensors can estimate the generated joint torques. %\cite{Nori2015iCub}.
% Instead, for hydraulic actuation system a pressure sensor can be used to estimate the generated torque.  
% The dynamics of a joint is subject to different types of friction, 
The torque control of the robot joints is more challenging because of the dynamics of the joints which is subject to friction and the mechanical power transmission from the motor to the joint shaft.
On the other side, compliance control of the joints allows for more robust locomotion and a safer interaction of the robot with the humans and the environment.
For example, ankle joint torque control allows for conforming the foot to the ground in case of small obstacles or mismatch between the ground slope and its estimation.
However, the compliance control with only joint torques may lead to poor velocity or position tracking, therefore a mixture of them is proposed in the feedback and feed-forward terms of the joint controller in \cite{johnson2017team, kuindersma2016optimization, cisneros2020inverse}.


\subsubsection{State Estimator}
Given the robot model, the state estimator uses the sensory information to estimate the robot's state, i.e., the floating base pose and velocity as well as the joint angles and velocities.
For the estimation, either proprioceptive sensors (i.e., joint encoders and IMU sensor attached to a robot link) or a combination of proprioceptive and exteroceptive sensors (such as cameras, GPS) are employed.
% However, the use of exteroceptive might be limiting specially in indoor unstructured and dynamic environments \cite{rotella2014state}.
When only proprioceptive sensors are used, a common approach is to assume that at each time instant at least one of the robot links is in contact with the ground, therefore the frame attached to the contact link has zero velocity and no slippage. With this assumption and taking into account the floating base frame pose in the kinematic chain, one can estimate the floating base velocity given the joints velocity vector. However, the error of estimation is propagated over time due to kinematic modeling errors. %Hence, 
To enhance the accuracy and limit the uncertainty of state estimation endowed with the odometry, IMU measurements are fused in the estimation process \cite{rotella2014state, bloesch2013state}. %cisneros2020lyapunov}.
Nevertheless, exploiting only the proprioceptive sensors does not lead to observability in the yaw axis (parallel to gravity vector) and the absolute position of the robot \cite{bloesch2013state}; thereby exteroceptive sensors can facilitate to overcome this difficulty.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%% WB CONTROL %%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Challenges and Limitations}

\subsection{Desiderata: Unified Motion Planning and Control}
\label{sec:ControlDesiderata}
% \todo[inline]{Luigi:I'd change this with a less confusing title. Since we already talked about simplified model based planner + stabilizer, here I would use a title that gives the idea we are now considering the whole robot model or more complex models. If I understood correctly}
% \label{sec:MotionPlanning}

% \textcolor{blue}{The composition of \textit{Path and Footstep Planner} and \textit{Stabilizer} with a unifying approach as a single control problem is known as \textit{Motion Planning and High-level Controller} in the literature which will be discussed later in Section \ref{sec:MotionPlanning}.}

% Sections \ref{sec:PathandFootstepPlanner} and  \ref{sec:Stabilizer}
Sections \ref{sec:controllerArchitecture} described the attempts to address the humanoid robot motion planning and control problem separately, i.e., dividing the problem into sub-problems and using the simplified models of the robot. Although this approach is computationally efficient, it is limiting due to the adopted simplifying assumptions. For example, the LIPM and fixed robot CoM height assumptions do not allow for agile motions where the robot angular motion is paramount; DCM-ZMP based stabilizers assumes there is always at least one contact point with no slippage between the robot and environment, contradicting to agile tasks such as jumping; it does not allow for generating human-like coordinated natural motions.
% especially about even terrains. 
% In case the robot should act on uneven terrain or in real-world scenarios with an unstructured environment, the robot needs to interact with its environment in a more complex fashion in order to perform agile actions and perform the given task.
% While in the previous section, different researchers in the literature tried to address the humanoid robot motion planning and control with the divide and conquer strategy, i.e., divide the problem into a number of sub-problems, and the simplified models of the robot are used in order to plan the robot motion and stabilize the system. However computationally efficient, that approach is limiting based on simplifying assumptions that are made in case the robot should act on uneven terrain and in real-world scenarios where the environment is unstructured and the robot needs to interact with its environment or perform agile actions. 
An alternative approach to solve the motion planning and control problem is to use the whole-body dynamics in the planning and control level, i.e., trying to solve the two problems simultaneously by identifying an optimization problem.
However, it is a non-linear and non-convex optimization problem with large input and state spaces, therefore it is computationally demanding and the optimization may suffer from local minima.

In recent years, %other communities among which
biomechanics, animation, and learning communities tried to address the problem of whole-body coordinated motion planning as well.
One major underlying component of the human-like coordinated motion is the control of the rotational motion and angular momentum for different tasks \cite{herr2008angular}.
To this goal, an \textit{angular excursion} index has been introduced by \cite{zordan2014control} relating the whole-body orientation, angular velocity, and centroidal angular momentum. When this idea integrates with linear momentum, it enables highly agile motion with considerable rotational behaviors \cite{Kuindersma2020Youtube, zordan2014control}. % and pose-tracking


To overcome the computational complexity of the trajectory optimization problem in multi-contact scenarios, \cite{lin2019efficient} suggested using a neural network for predicting the dynamic evolution of the centroidal dynamics over transition phases.
Instead in \cite{peng2018deepmimic}, the authors have proposed a deep reinforcement learning (RL) approach to learn the necessary skills for animated characters by using motion capture data. In their approach, they learn the control policy in order to maximize the reward associated with motion imitation as well as task objectives.
Following that, an iterative RL-based approach has been experimented on a real biped robot in \cite{xie2019iterative}.


% \iffalse
% % A possibility is to adopt a trade-off solution between simplified control approaches and whole-body dynamical motion planning, by considering the centroidal dynamics and the whole-body kinematics of the robot at the planning level and using this information to find feasible the low-level joint commands \cite{dai2014whole}.
% Another possible trade-off solution between simplified and whole-body motion planning appraches is to adopt the centroidal dynamics and the whole-body kinematics of the robot at the planning level and using these information to find feasible low-level joint commands \cite{dai2014whole}.
% This approach 
% %can find feasible trajectories, benefiting
% benefits from both the centroidal dynamics constraints and whole-body kinematics in the collision avoidance and reachability computations.
% \iffalse
% \textcolor{red}{Given the centroidal dynamics in \eqref{eq:eulermomentum} and whole-body kinematics, the whole-body motion planning and control problem is defined with the following objective function \cite{dai2014whole}:
% \begin{equation}
% \begin{array}{c}
% % \begin{matrix}
%  \underset{ \Gamma(j) } {\text{arg~min}}
%  \sum_{j=1}^{N} \{ \|\bm{q}(j) -\bm{q}^{d}(j)\|^2_{ \bm{Q}_s} + \| {\bm{\nu}}(j) \|^2_{ \bm{Q}_{{\nu}}} + \\
% \quad\quad \| \ddot{\bm{x}}_{\mathcal{COM}}(j) - \ddot{\bm{x}}^d_{\mathcal{COM}}(j) \|^2_{\bm{Q}_{COM}} + \\ \| \dot{\bm{k}}(j) - \dot{\bm{k}}^d \|^2_{\bm{Q}_{k}} + \\
% \sum_{i=1}^{c} ( \| \bm{f}_i(j) \|^2_{\bm{Q}_F} + \| \bm{f}_i(j) \|_{\bm{Q}'_F})\}\delta t(j),\\
% % s.t. 
% %           \quad\quad \bm{\dot{h}} - \bm{f}(\bm{q}, \bm(\nu), \bm{\dot{\nu}}, \bm{\tau})=\bm{0},\\ \quad\quad \bm{g}((\bm{x}, \bm{u})) \le \bm{0},\\ 
% %           \quad\quad \bm{h}((\bm{x}, \bm{u})) = \bm{0},
% % \end{matrix} 
% % \underset{\begin{subarray}{c}\bm{q}(j), \bm{\nu}(j), dt(j), {\bm{x}}^d_{\mathcal{COM}}(j), \\ \dot{\bm{x}}^d_{\mathcal{COM}}(j), \ddot{\bm{x}}^d_{\mathcal{COM}}(j), \\ \bm{h}(j), \dot{\bm{h}}(j), \bm{c}_i(j), \bm{F}_i(j) \end{subarray}} {\text{arg~min}}~ \sum_{j=1}^{N} (\|\bm{q}(j) -\bm{q}^{d}(j)\|^2_{ \bm{Q}_s} + \| {\bm{\nu}}(j) \|^2_{ \bm{Q}_{{\nu}}} + \\
% % \| \ddot{\bm{x}}_{\mathcal{COM}}(j) - \ddot{\bm{x}}^d_{\mathcal{COM}}(j) \|^2_{\bm{Q}_{COM}} + \| \dot{\bm{k}}(j) - \dot{\bm{k}}^d \|^2_{\bm{Q}_{k}} + \\
% % \sum_{i=1}^{c} ( \| \bm{F}_i(j) \|^2_{\bm{Q}_F} + \| \bm{F}_i(j) \|_{\bm{Q}'_F}))dt(j)
% \end{array}
% \label{eq:wbmpcDesiderata}% whole body motion planning & control Desiderata
% \end{equation}
% where $\Gamma(j)$ is the set of decision variables, i.e., $ \bm{q}(j)$ the robot configuration, $\bm{\nu}(j)$ the velocity vector, $\delta t(j)$ the knot point (points joining two polynomial segments in the optimization process), ${\bm{x}}^d_{\mathcal{COM}}(j), \dot{\bm{x}}^d_{\mathcal{COM}}(j), \ddot{\bm{x}}^d_{\mathcal{COM}}(j)$ the CoM motion vectors, $\bm{h}(j)$ the momentum, $\dot{\bm{h}}(j)$ rate of change of momentum, and $\bm{c}_i(j), \bm{f}_i(j)$ the $i$'th contact point and wrench values.
% In this formula, the first term of the objective function is related to the joint angle errors, the second term regularizes the joint velocities, the third term is related to the CoM motion error, the fourth term penalizes the rate of change of angular momentum, and the last two terms penalize the external contact forces and promote the sparsity of the external contact forces acting on the robot, respectively.
% % \todo{Luigi: respectively?}
% % $\bm{f}_{j}$ in this formula is the vector of all the external wrenches acting on the robot.
% This equation can be followed by an inverse dynamics formulation to compute the robot joint torques.
% Following \eqref{eq:wbmpcDesiderata}, a inverse dynamics formulation computes the robot joint torques.}

% \textcolor{red}{
% The trajectory optimization problem described in \eqref{eq:wbmpcDesiderata} is subject to constraints.
% The first set of constraints is related to the dynamics of the system at each %\todo[]{Luigi: what do you mean by knot point?} \todo[]{Kourosh: described in previous paragraph!} 
% knot point, including the centroidal dynamics, the momentum vector of the system, the time evolution of the joint angles and velocities, and COM motion. 
% %\todo[inline]{Luigi:I don't get this sentence. "They" refers to constraints. their derivate is already given?}
% These constraints are found by the time integration of their derivatives.
% % Using the robot states and forward kinematics, one can compute the COM position and the contact points of the robot.
% The second set of constraints are related to the inequality constraints on the configuration and velocity vectors, and the contact points and wrenches can be applied. When solving the optimization problem, the contact constraints are transformed into a set of complementary constraints as explained in \cite{posa2014direct, dai2014whole}.}
% \fi
% \textcolor{blue}{ %MPC
% % It is a suite of optimization-based control techniques applied to dynamical systems. \cite{dai2014whole}
% A common approach in the literature similar to \cite{dai2014whole} is to employ MPC for the purpose.
% MPC are a suite of optimal control techniques that optimize an objective function based on a predicted evolution of the system states in the future \cite{borrelli2017}, therefore a model of robot is needed.}
% % In a linear case, the prediction model is:
% % \begin{equation}
% % \begin{cases} 
% % \bm{x}_{k+1}=\bm{A}\bm{x}_{k}+\bm{B}\bm{u}_{k} \\
% % \bm{y}_{k}=\bm{C}\bm{x}_{k},
% % \end{cases}
% % \label{eq:mpc1}
% % \end{equation}
% % where $\bm{x}_k$, $\bm{u}_k$ and $\bm{y}_k$ are respectively the state, the input and the output of the system at time $k$.
% % An approach to relating the input and the current state vector can be formulated as:
% % \begin{equation}
% % \bm{x}_{k}=\bm{A}^k\bm{x}_{0}+\sum_{j=0}^{k-1}\bm{A}^j\bm{B}\bm{u}_{k-1-j}.
% % \label{eq:mpc2}
% % \end{equation}
% % The goal is to solve the following optimization problem, finding the optimal sequence of control inputs:
% % \begin{equation}
% % \begin{array}{c}
% % \underset{\bm{u}_0, ..., \bm{u}_{N-1} }{\text{arg~min}}~\bm{x}_N^T\bm{P}\bm{x}_N+\sum_{k=0}^{N-1}\bm{x}_k^T\bm{Q}\bm{x}_k+\bm{u}_k^T\bm{R}\bm{u}_k,\\
% %  s.t. 
% %           \quad\quad \bm{\dot{x}} - \bm{f}(\bm{x}, \bm{u})=\bm{0},\\ \quad\quad \bm{g}((\bm{x}, \bm{u})) \le \bm{0},\\ 
% %           \quad\quad \bm{h}((\bm{x}, \bm{u})) = \bm{0},
% % \end{array}
% % \label{eq:mpc3}
% % \end{equation}
% % where $\bm{R}$ is a positive definite matrix and $\bm{Q}$ and $\bm{P}$ are positive semi-definite matrices. 
% % Moreover, the MPC problem is accompanied by a set of constraints including the robot dynamics constraint (the first constraint in \eqref{eq:mpc3}), inequality constraints such as joint position, velocity and torque limits, contact unilaterality and friction cone constraints, and finally equality constraints such as  non-sliding contact constraints.
% %%%%%

% The optimal control problem is solved by transforming it into an algebraic nonlinear programming problem, namely through a transcription process \cite{kelly2017introduction, rao2009survey}.
% To do that, two categories of shooting methods and direct methods are utilized in the literature. While the shooting method searches for input variable values and uses the forward simulation results to compute the cost of trajectory, the direct method finds the input and state variable simultaneously without explicit simulation.
% The multiple shooting method blends these two approaches together as explained in \cite{posa2014direct}.
% However, the main limitation of optimal control approaches, is specific MPC, for humanoid robot control is the computational cost of solving the optimization problem.
% Therefore, the use of them in real-time is typically not straightforward and it is usually convenient to recur to a simplified prediction model. More recently, \cite{mastalli20crocoddyl} attempted to address the computational time challenge by using variations of differential dynamic programming approach.
% The trajectory optimization problem is subject to constraints.
% The first set of constraints is related to the dynamics of the robotic system,
% % at knot points (points joining two polynomial segments in the optimization process),
% including the centroidal dynamics, the momentum vector of the system, the time evolution of the joint angles and velocities, and CoM motion. 
% %\todo[inline]{Luigi:I don't get this sentence. "They" refers to constraints. their derivate is already given?}
% % These constraints are found by the time integration of their derivatives.
% % Using the robot states and forward kinematics, one can compute the COM position and the contact points of the robot.
% The second set of constraints are related to the inequality constraints on the configuration and velocity vectors, and the contact points and wrenches.
% When solving the optimization problem, the contact constraints are transformed into a set of complementary constraints as explained in \cite{posa2014direct, dai2014whole}.
% %%%%%

% \fi

% \iffalse

% %
% %
% %%%
% %%%%
% %%
% %
% %%%%%
% Another possible trade-off solution between simplified and whole-body motion planning appraches is to adopt the centroidal dynamics and the whole-body kinematics of the robot at the planning level and using these information to find feasible low-level joint commands \cite{dai2014whole}.
% This approach benefits from both the centroidal dynamics constraints and whole-body kinematics in the collision avoidance and reachability computations.


% A common approach in the literature similar to \cite{dai2014whole} is to employ MPC for the purpose.
% MPC are a suite of optimal control techniques that optimize an objective function based on a predicted evolution of the system states in the future \cite{borrelli2017}, therefore a model of robot is needed.
% The optimal control problem is solved by transforming it into an algebraic nonlinear programming problem, namely through a transcription process \cite{kelly2017introduction, rao2009survey}.
% To do that, two categories of shooting methods and direct methods are utilized in the literature. While the shooting method searches for input variable values and uses the forward simulation results to compute the cost of trajectory, the direct method finds the input and state variable simultaneously without explicit simulation.
% The multiple shooting method blends these two approaches together as explained in \cite{posa2014direct}.
% However, the main limitation of optimal control approaches, is specific MPC, for humanoid robot control is the computational cost of solving the optimization problem.
% Therefore, the use of them in real-time is typically not straightforward and it is usually convenient to recur to a simplified prediction model. More recently, \cite{mastalli20crocoddyl} attempted to address the computational time challenge by using variations of differential dynamic programming approach.}
% \textcolor{blue}{ 
% The trajectory optimization problem is subject to constraints.
% The first set of constraints is related to the dynamics of the robotic system,
% % at knot points (points joining two polynomial segments in the optimization process),
% including the centroidal dynamics, the momentum vector of the system, the time evolution of the joint angles and velocities, and CoM motion. 
% %\todo[inline]{Luigi:I don't get this sentence. "They" refers to constraints. their derivate is already given?}
% % These constraints are found by the time integration of their derivatives.
% % Using the robot states and forward kinematics, one can compute the COM position and the contact points of the robot.
% The second set of constraints are related to the inequality constraints on the configuration and velocity vectors, and the contact points and wrenches.
% When solving the optimization problem, the contact constraints are transformed into a set of complementary constraints as explained in \cite{posa2014direct, dai2014whole}.
% %%%%%

% %%%%%\%iffa%%%%l%se
% Furthermore, the inequality constraints on the configuration and velocity vectors, and the contact points and wrenches can be applied by:
% \begin{equation}
% \begin{array}{c}
% \bm{q} \in \mathcal{Q},~ \bm{\nu} \in \mathcal{N},~ \bm{f}_i \in \mathcal{F}_i, \bm{c}_i(j) \in \mathcal{S}_i(j) ,
% \end{array}
% \label{eq:constraintsDesiderata}% whole body motion planning & control Desiderata
% \end{equation}
% where $\mathcal{Q}$ and $\mathcal{N}$ are the admissible set of postures and velocities and $\mathcal{F}_i$ the admissible set of contact wrenches for each contact point, and $\mathcal{S}_i(j)$ is the admissible set of contact regions at time instant $j$ for each contact $i$.

% In order to include the contact constraints, three points should be addressed, i.e. the sequence of contacts, the location of the contacts, and the time instant the contact is established. For simplicity, rigid contacts and non-sliding contacts (rather than compliant and sliding contacts) are considered.
% However, automatically identifying the contact sequences can combinatorially explode as the number of contact modes increases.
% For simplicity, we assume at each contact point the reaction torque is zero, and $F$ represents only the contact force.
% In \cite{posa2014direct}, the contact constraints including the contact wrench and contact distance are transformed into a set of complementary constraints as:
% \begin{subequations} \label{eq:ContactConstraints}
% \begin{align}
% & \bm{\phi}_i(\bm{q(j)}) \geq 0, \label{eq:ContactConstraints:A}\\
% & \bm{F}^n_i \geq 0,\label{eq:ContactConstraints:B}\\
% &  \forall i: \bm{\phi}_i\bm{(q(k))} \bm{F}_i=0,\label{eq:ContactConstraints:C}\\
% &  \forall i: \bm{F}^n_i ( (c_j(i)- c_j(i-1) )\bm{t}_x)=0,\label{eq:ContactConstraints:D}\\
% &  \forall i: \bm{F}^n_i ( (c_j(i)- c_j(i-1) )\bm{t}_y)=0,\label{eq:ContactConstraints:E}
% \end{align}
% \end{subequations}
% the first term of the constraint equation declares the distance $\bm{\phi}_i(\bm{q(j)})$ between the robot $i$'th contact point $c_i$ and the contact surface $\mathcal{S}_i$ should be positive, \eqref{eq:ContactConstraints:B} represents the unilateral constraint of the normal of the reaction forces, \eqref{eq:ContactConstraints:C} represents the complementary constraint, thereby the contact force is not equal to zero if and only if the distance $\bm{\phi}_i(\bm{q(j)})$ is set to zero (the bodies are in contact). 
% The last two terms of \eqref{eq:ContactConstraints} adopted from \cite{dai2014whole} indicate the non-sliding constraint along the contact surface when the contact force is not zero. $\bm{t}_x$ and $\bm{t}_y$ indicate the orthogonal unit vectors tangential to the contact surface.
% % \textcolor{blue}{Finally, in the literature, different choices of task objectives and constraints for the whole-body motion planning and control have been suggested.}
% % to reach in the cost function in \eqref{}, such as desired base frame orientation \cite{eq:wbmpcDesiderata}, or other set of constraints such as foot height and orientations constraints \cite{}.
% \fi


% % other constraints such as base orientation, 







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Another possible trade-off solution between simplified and whole-body motion planning approaches is to adopt the centroidal dynamics and the whole-body kinematics of the robot at the planning level and using this information to find feasible low-level joint commands \cite{dai2014whole}.
This approach benefits from both the centroidal dynamics constraints and whole-body kinematics in the collision avoidance and reachability computations.
A common approach in the literature, similar to \cite{dai2014whole}, is to employ MPC for the purpose.
MPC are a suite of optimal control techniques that optimize an objective function based on a predicted evolution of the system states in the future \cite{borrelli2017}, therefore a model of the robot is needed.
The optimal control problem is solved by transforming it into an algebraic nonlinear programming problem, namely through a transcription process \cite{kelly2017introduction, rao2009survey}.
To do that, two categories of shooting methods and direct methods are utilized in the literature. While the shooting method searches for input variable values and uses the forward simulation results to compute the cost of trajectory, the direct method finds the input and state variable simultaneously without explicit simulation.
The multiple shooting method blends these two approaches as explained in \cite{posa2014direct}.
However, the main limitation of optimal control approaches, in specific MPC, for humanoid robot control is the computational cost of solving the optimization problem.
Therefore, the use of them in real-time is typically not straightforward and it is usually convenient to recur to a simplified prediction model. More recently, \cite{mastalli20crocoddyl} attempted to address the computational time challenge by using variations of differential dynamic programming approach.
Finally, the trajectory optimization problem is subject to constraints.
The first set of constraints is related to the dynamics of the robotic system, including the centroidal dynamics, the momentum vector of the system, the time evolution of the joint angles and velocities, and CoM motion. 
The second set of constraints are related to the inequality constraints on the configuration and velocity vectors, and the contact points and wrenches.
When solving the optimization problem, the contact constraints are transformed into a set of complementary constraints as explained in \cite{posa2014direct, dai2014whole}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> sections/9-DiscussionOpenProblems.tex <==
\section{Discussions}
\label{sec:Discussion}

\iffalse
Future applications of teleoperated humanoid robots are very promising but further progress is required to employ these robots in real world scenarios. Major improvements have been achieved in the past in the context of the DRC, and great expectations are now on the technological advancements that will emerge from the ongoing global competition ANA AVATAR XPRIZE.


After having analyzed the potential impact of employing teleoperated humanoid robots in different application scenarios (Section \ref{sec:Applications}), let us briefly analyze the current limitations of such technologies. First, despite being attractive because of their anthropomorphism and potential to operate in environments designed for humans, humanoid robots are still expensive and not affordable for many industries and research institutes.
So far, this inconvenience has strongly limited their study to a restricted robotics community.
% , being employed exclusively in the research field. 
Moreover, very often either the robot hardware or the underlying control software (or both) are not designed to comply with control failures, loss of balance or wrong interactions with the environment, which can lead to costly breakage. 

In the sensoristic field, instead, a lot of progress has been made in the last decade (Section \ref{sec:HumanSensoryMeasurementsDevices}). A heterogeneous combination of tracking and haptic sensors now allow teleoperated robots to operate more effectively in their environments, however more improvement is expected in HRI in order to allow the robot to perform richer interactions with  both operators and bystanders. The few teleoperation-related work that addressed this topic \cite{peer2008,evrard2009}, have been limited to studying the interaction at the level of the robot's upper limbs exclusively; an extension to a whole-body level has yet to be investigated.

A current major limitation in robot teleoperation, particularly in space applications, is the unavoidable use of non-ideal communication networks.
Despite being very promising for their intrinsic binding between human and robot state, especially sought in telexistence, bilateral systems struggle in the presence of communication delays, which strongly reduce the transparency of the system (Section \ref{sec:bilateral}). Master-slave humanoid robot systems present less instability issues in the presence of delay, but existing compensation approaches \cite{smith2010,clarke2008} cannot tolerate delays higher than 200 milliseconds yet.

A final challenge in humanoid teleoperation is to build a system that can be easily mastered by non-expert users. State of the art work, do not often consider any usability assessment or carry out any user study, strongly relying on the expertise and training of a single human operator. In this perspective, we hope Section \ref{sec:EvaluationMetrics} could help the reader in identifying the key points and right evaluation metrics for deploying a teleoperation system that meets the user's needs.

\fi
